Model-Free DRL Control for Power Inverters: From Policy Learning to Real-Time Implementation via Knowledge Distillation

In response to the trade-off between control performance and computational burden hindering the deployment of Deep Reinforcement Learning (DRL) in power inverters, this paper presents a novel model-free control framework leveraging policy distillation. To handle the convergence instability and steady-state errors inherent in model-free agents, an error energy-guided hybrid reward mechanism is established to theoretically constrain the exploration space. More specifically, an adaptive importance weighting mechanism is integrated into the distillation architecture to amplify the significance of fluctuation regions, ensuring high-quality transfer of transient control logic by mitigating the observational bias dominated by steady-state data. This approach efficiently compresses the heavy DRL policy into a lightweight neural network, retaining the desired control performance while overcoming the computational bottleneck during deployment. The proposed method is validated through a hardware-based kilowatt-level experimental platform. Experimental comparison results with traditional methods demonstrate that the proposed technique reduces inference time to the microsecond level and achieves superior transient response speed and parameter robustness.

==> paper3/translate/translate.tex <==
\section{引言}
随着可再生能源、储能和电动汽车的接入，电力系统正朝着智能化方向发展。分布式能源的整合和各种商业模式的实施使得人的参与和互动变得越来越重要。因此，将电力用户行为纳入电力系统决策回路显得尤为必要。电力系统中的用户行为包括用电行为、产电行为和电动汽车充放电行为，这些行为对电力系统的稳定性和经济性有着越来越显著的影响。因此，构建不同时间、空间和场景的用户行为模型，以描述各类用户行为特征，为规划、需求侧资源协同优化和电力交易提供理论和技术支持变得越来越重要。用电行为建模是电力系统用户行为分析的重要组成部分。通过分析用电行为可以描述各类用户的用电特征，最终提高用电效率，为电网运行规划提供帮助[3]，[4]。
1.With the integration of renewable energy, energy storage, and electric vehicles, the power system is evolving towards intelligence. The integration of distributed energy resources and the implementation of various business models have made human participation and interaction increasingly important. Therefore, incorporating electricity user behavior into the decision-making loop of the power system is particularly necessary. User behavior in the power system includes electricity consumption, electricity generation, and electric vehicle charging and discharging behaviors, which have an increasingly significant impact on the stability and economics of the power system. Therefore, it is becoming more and more important to build user behavior models for different time, space, and scenarios to describe various user behavior characteristics, providing theoretical and technical support for planning, demand-side resource optimization, and power trading. Modeling electricity consumption behavior is an important component of power system user behavior analysis. By analyzing electricity consumption behavior, various user's electricity consumption characteristics can be described, ultimately improving electricity efficiency and assisting in power grid operation and planning.
2.As renewable energy, energy storage, and electric vehicles become part of the power grid, the electricity system is moving towards greater intelligence. The integration of distributed energy sources and various business models highlights the increasing importance of human involvement and interaction. Therefore, it is crucial to incorporate user behavior into the decision-making processes of the electricity system. User behavior in the power system includes electricity usage, electricity generation, and electric vehicle charging and discharging patterns, all of which have a growing impact on the stability and cost-effectiveness of the electricity system. Consequently, developing models that describe different user behaviors in terms of time, space, and scenarios is becoming increasingly vital. These models provide the theoretical and technical foundation for planning, optimizing demand-side resources, and facilitating electricity trading activities. Modeling electricity usage behavior is a key aspect of analyzing user behavior in the power system. By studying electricity consumption behavior, we can identify and understand various user consumption patterns, ultimately enhancing energy efficiency and supporting effective power grid operation and planning.
3，As renewable energy, energy storage, and electric vehicles are integrated into the power grid, the electricity system is advancing towards enhanced intelligence. The incorporation of distributed energy sources and diverse business models underscores the growing importance of human engagement and interaction. Hence, including user behavior in the decision-making loop of the electricity system is increasingly imperative. User behavior within the power system encompasses electricity consumption, generation, and electric vehicle charging/discharging actions, with their impact on system stability and cost efficiency becoming more pronounced. Thus, the development of user behavior models across different time frames, locations, and scenarios is progressively crucial. These models offer the necessary theoretical and technical support for planning, optimizing demand-side resources, and facilitating electricity transactions. Modeling electricity consumption behavior serves as a crucial component in understanding user behavior within the power system. By analyzing electricity usage patterns, various characteristics can be identified to improve energy efficiency and aid in effective power grid operations and planning.

目前，电力用户行为建模主要包括统计分析、数据挖掘、随机建模和代理模型等方法。统计分析是电力用户行为建模中最传统且广泛应用的方法，通过统计技术分解用户电力消费行为，提取用户行为电力趋势、周期性和节假日影响特征。【Wu & Li, 2019】虽然这些方法简单且解释性好，但在处理复杂和非线性行为时效果有限。数据挖掘利用大数据技术，通过聚类或者深度学习等方法挖掘用户大数据中的准确信息，有效分析用户的电力消费行为。【Chuang et al., 2021】。该方法可以处理大规模数据并发现隐藏模式，但需要大量计算资源和高质量数据。电力用户行为具有高度随机性，因此随机建模方法在电力用户行为建模中应用广泛。这类方法利用随机模型如马尔可夫模型和Copula函数描述用户行为的随机性和波动性【Meidani & Ghanem, 2013】。它们擅长处理不确定性，但模型复杂且参数敏感。近年来，基于代理的建模方法在处理电力用户行为的复杂性和动态性方面呈现出显著优势。通过多种代理建模技术，如多层代理模型、强化学习和博弈理论，可以有效地模拟和预测用户的电力消费行为。但是上述方法缺少对人类的复杂角色和心理的描述。
1. Currently, electricity user behavior modeling mainly includes methods such as statistical analysis, data mining, stochastic modeling, and agent-based modeling. Statistical analysis is the most traditional and widely used method in electricity user behavior modeling. It decomposes user electricity consumption behavior using statistical techniques to extract characteristics such as user behavior trends, periodicity, and holiday effects. Although these methods are simple and have good interpretability, their effectiveness is limited when dealing with complex and nonlinear behaviors. Data mining utilizes big data technology to extract accurate information from user big data through methods like clustering or deep learning, effectively analyzing user electricity consumption behavior. This method can handle large-scale data and uncover hidden patterns but requires substantial computational resources and high-quality data. Electricity user behavior is highly stochastic, hence stochastic modeling methods are widely applied in electricity user behavior modeling. These methods use stochastic models such as Markov models and Copula functions to describe the randomness and variability of user behavior. They excel in handling uncertainty but have complex models and are sensitive to parameters. In recent years, agent-based modeling methods have shown significant advantages in addressing the complexity and dynamism of electricity user behavior. Through various agent modeling technologies, such as multi-agent models, reinforcement learning, and game theory, user electricity consumption behavior can be effectively simulated and predicted. However, these methods lack descriptions of the complex roles and psychology of humans.

2. Currently, the modeling of electricity user behavior mainly includes methods such as statistical analysis, data mining, stochastic modeling, and agent-based modeling. Statistical analysis is the most traditional and widely used method in modeling electricity user behavior. By using statistical techniques to break down user electricity consumption behavior, it extracts characteristics such as user behavior trends, periodicity, and holiday impacts. Although these methods are simple and have good interpretability, their effectiveness is limited when dealing with complex and nonlinear behaviors. Data mining utilizes big data technology to extract accurate information from user big data through methods such as clustering or deep learning, effectively analyzing user electricity consumption behavior. This method can handle large-scale data and uncover hidden patterns but requires significant computational resources and high-quality data. Due to the high stochastic nature of electricity user behavior, stochastic modeling methods are widely used. These methods leverage stochastic models such as Markov models and Copula functions to describe the randomness and variability of user behavior. They are good at handling uncertainty but have complex models and are sensitive to parameters. In recent years, agent-based modeling methods have demonstrated significant advantages in addressing the complexity and dynamism of electricity user behavior. Through various agent modeling techniques, like multi-agent models, reinforcement learning, and game theory, user electricity consumption behavior can be effectively simulated and predicted. However, these methods lack a description of the complex roles and psychology of humans.

3. Currently, models of electricity user behavior include statistical analysis, data mining, stochastic modeling, and agent-based modeling. Statistical analysis is the traditional and commonly used method in electricity user behavior modeling, extracting user electricity consumption behavior characteristics such as trends, periodicity, and holiday impacts. Although simple and interpretable, these methods may have limited effectiveness with complex and nonlinear behaviors. Data mining, utilizing big data technology, extracts accurate information from user big data through methods like clustering or deep learning for analyzing electricity consumption behavior. This method handles large-scale data and uncovers hidden patterns but requires substantial computational resources and high-quality data. Given the high stochastic nature of electricity user behavior, stochastic modeling methods are widely applied, using models like Markov models and Copula functions to describe behavior randomness and variability. While effective in handling uncertainty, these models are complex and parameter-sensitive. Agent-based modeling methods have shown significant advantages in addressing the complexity and dynamics of electricity user behavior in recent years, using technologies like multi-agent models, reinforcement learning, and game theory for simulating and predicting user electricity consumption behavior. However, these methods lack descriptions of the intricate roles and psychology of humans.

大语言模型（Large Language Models, LLMs）和生成式代理（Generative Agents）的进步正在快速改变用户行为建模的方式。生成式代理能够通过自然语言理解和生成，精确模拟复杂的人类行为和决策过程，提供更高的建模精度和灵活性。Park等人（2023）提出了生成式代理的概念，能够模拟人类的日常行为，如醒来、做饭和上班，并在交互式沙盒环境中展示逼真的个体和社会行为【Park et al., 2023】。Lyfe代理结合大语言模型，模拟复杂的社交行为，通过自然语言处理实现低成本的实时响应，在多代理场景中展示自我动机和社会推理能力。Xu和Zhang（2023）探讨了大语言模型在模拟学生学习行为中的应用，证明这些虚拟学生能够反映真实的学习模式和行为【Xu & Zhang, 2023】。这些模型通过大语言模型实现了人类行为的准确模拟。同样，电力用户行为受到用户特征和心理因素的影响，因此，引入基于大语言模型的生成式代理进行电力用户行为建模，可以提高准确性，支持电力预测和决策。
1. The advancements in Large Language Models (LLMs) and Generative Agents are rapidly changing the way user behavior modeling is conducted. Generative Agents can accurately simulate complex human behaviors and decision-making processes through natural language understanding and generation, providing higher modeling accuracy and flexibility. Park et al. (2023) introduced the concept of Generative Agents, capable of simulating human daily activities like waking up, cooking, and going to work, showcasing realistic individual and social behaviors in interactive sandbox environments. Lyfe agents, combining Large Language Models, simulate complex social behaviors and achieve low-cost real-time responses through natural language processing, demonstrating self-motivation and social reasoning abilities in multi-agent scenarios. Xu and Zhang (2023) explored the application of Large Language Models in simulating student learning behaviors, proving that these virtual students can reflect real learning patterns and behaviors. These models achieve accurate simulation of human behaviors through Large Language Models. Similarly, as electricity user behavior is influenced by user characteristics and psychological factors, introducing Generative Agents based on Large Language Models for modeling electricity user behavior can enhance accuracy, support power forecasting, and decision-making.

2. The rapid evolution of Large Language Models (LLMs) and Generative Agents is fundamentally altering the landscape of user behavior modeling. Generative Agents excel in accurately simulating complex human behaviors and decision-making processes through natural language understanding and generation, offering increased modeling precision and adaptability. Park et al. (2023) introduced the concept of Generative Agents capable of mimicking various human daily activities such as waking up, cooking, and going to work, showcasing lifelike individual and social behaviors within interactive sandbox environments. By leveraging Large Language Models, Lyfe agents simulate intricate social behaviors efficiently, enabling real-time responses at low costs through natural language processing, showcasing self-motivation and social reasoning abilities in complex multi-agent scenarios. Xu and Zhang (2023) explored the utilization of Large Language Models in modeling student learning behaviors, showcasing the ability of virtual students to mirror authentic learning patterns and behaviors. These models achieve precise human behavior simulation through the use of Large Language Models. Likewise, given that electricity user behavior is influenced by user traits and psychological elements, incorporating Large Language Model-based Generative Agents for electricity user behavior modeling can enhance accuracy, facilitate power prediction, and support decision-making processes.

3. The rapid progress of Large Language Models (LLMs) and Generative Agents is swiftly revolutionizing the approach to user behavior modeling. Generative Agents have the capacity to intricately simulate complex human behaviors and decision-making processes through natural language comprehension and generation, providing heightened modeling precision and adaptability. Park et al. (2023) introduced the concept of Generative Agents that can replicate human daily activities such as waking up, cooking, and going to work, presenting authentic individual and social behaviors within interactive sandbox environments. Through the integration of Large Language Models, Lyfe agents simulate elaborate social behaviors, enabling cost-effective real-time responses via natural language processing, showcasing self-motivation and social reasoning capabilities within multi-agent settings. Xu and Zhang (2023) delved into the application of Large Language Models in simulating student learning behaviors, demonstrating that these virtual students can mirror real learning patterns and behaviors accurately. These models attain precise simulation of human behavior through Large Language Models. Additionally, as electricity user behavior is influenced by user characteristics and psychological factors, the introduction of Generative Agents based on Large Language Models for electricity user behavior modeling can enhance accuracy, support power forecasting, and decision-making.

世界模型
world model



针对上述问题，本文提出了一种基于生成式代理的电力用户行为模型，用于模拟和分析电力用户行为。
智能涌现社会带来什么？自己模型：
To solve these problems, this paper proposes a power user behavior model based on generative agent, which is used to simulate and analyze power user behavior.What does an intelligent emergent society bring?Own model:

The main contributions are as follows:
\begin{itemize}
    \item \ A power user behavior model based on generative agent is proposed.
    \item \ The power user behavior of generative agent is described from four dimensions of time, space, energy and price.
    \item \ A generative agent simulation method based on statistical information enhancement is proposed.
\end{itemize}



\section{Generative Agent}


### Mathematical description of a generative agent

生成式代理（Generative Agents）是一种能够模拟人类行为和决策的智能系统，具备记忆、检索、反思和交互能力。以下是生成式代理的数学描述，包括其核心组件和功能。
1. Generative Agents are intelligent systems capable of simulating human behaviors and decision-making, with the ability to remember, retrieve, reflect, and interact. The following is a mathematical description of Generative Agents, including their core components and functions.
2. Generative Agents are intelligent systems that can simulate human behaviors and decision-making, possessing the abilities of memory, retrieval, reflection, and interaction. Here is a mathematical description of Generative Agents, including their core components and functions.
3. Generative Agents are intelligent systems that can replicate human behaviors and decision-making, equipped with memory, retrieval, reflection, and interaction capabilities. The following is a mathematical depiction of Generative Agents, detailing their core components and functionalities.

\subsection{Memory Module}
生成式代理的记忆模块用于存储和管理历史信息。假设在时间 \( t \) 时，代理的记忆状态为 \( M_t \)，包含 \( N \) 条记忆条目，每条记忆条目 \( m_i \) 包含信息 \( I_i \) 和时间戳 \( t_i \)：
1. The memory module of a generative agent is employed to store and manage historical information. At time \( t \), the agent's memory state is \( M_t \), which comprises \( N \) memory entries, with each memory entry \( m_i \) containing information \( I_i \) and a timestamp \( t_i \).

2. The memory module of a generative agent is utilized for storing and managing historical information. At time \( t \), the agent's memory state is \( M_t \), containing \( N \) memory entries, where each memory entry \( m_i \) includes information \( I_i \) and a timestamp \( t_i \).

3. The memory module of a generative agent is used to store and maintain historical information. At time \( t \), the agent's memory state is \( M_t \), which consists of \( N \) memory entries. Each memory entry \( m_i \) contains information \( I_i \) and a timestamp \( t_i \).

\subsection{Retrieval Module}

检索模块用于从记忆中提取相关信息。假设有一个检索查询 \( q \)，代理需要从记忆 \( M_t \) 中找到与 \( q \) 最相关的记忆条目。相关性可以通过余弦相似度等方法计算：
1. The retrieval module is used to extract relevant information from memory. Assuming there is a retrieval query \( q \), the agent needs to find the memory entry in \( M_t \) that is most relevant to \( q \). The relevance can be calculated using methods such as cosine similarity.

2. The retrieval module is designed to extract relevant information from memory. Given a retrieval query \( q \), the agent is required to locate the memory entry in \( M_t \) that is most pertinent to \( q \). Relevance can be computed using methods like cosine similarity.

3. The retrieval module is responsible for retrieving pertinent information from memory. With a retrieval query \( q \) in place, the agent must identify the most relevant memory entry in \( M_t \). The degree of relevance can be determined using techniques such as cosine similarity.

\subsection{Reflection Module}

反思模块用于对记忆和当前状态进行反思，形成新的见解和决策。假设反思函数为 \( f_{\text{reflect}} \)，它接受当前记忆状态 \( M_t \) 和检索到的记忆条目 \( I^* \) 作为输入，并输出反思结果 \( R \)：
1. The reflection module is used to reflect on memory and the current state, forming new insights and decisions. Assuming the reflection function is \( f_{\text{reflect}} \), it takes the current memory state \( M_t \) and retrieved memory entry \( I^* \) as inputs, and outputs the reflection result \( R \).
2. The reflection module is employed to reflect on memory and the current state, leading to the generation of new insights and decisions. It operates with the reflection function \( f_{\text{reflect}} \), which takes the current memory state \( M_t \) and the retrieved memory entry \( I^* \) as inputs, and produces the reflection result \( R \).
3. The reflection module is utilized for pondering over memory and the current state to derive new insights and make decisions. Assuming the reflection function is \( f_{\text{reflect}} \), it takes the current memory state \( M_t \) and the retrieved memory entry \( I^* \) as inputs, and yields the reflection result \( R \).

\subsection{Interaction Module}

交互模块用于生成与用户或环境的互动响应。假设当前状态为 \( S_t \)，生成的响应为 \( A \)，交互函数为 \( f_{\text{interact}} \)：

生成的响应 \( A \) 可以是自然语言对话、行动计划或其他形式的输出。
通过这一循环过程，生成式代理能够持续地学习、反思和交互，从而模拟人类的行为和决策过程。该数学模型描述了生成式代理的核心功能和工作机制，为构建和研究智能代理系统提供了理论基础。
1. The role of the interaction module is to generate interactive responses to users or the environment. Assuming the current state is \( S_t \) and the generated response is \( A \), the interaction function is \( f_{\text{interact}} \).

2. The interaction module is designed to produce interactive responses to users or the environment. With the current state being \( S_t \) and the response generated as \( A \), the interaction function is \( f_{\text{interact}} \).

3. The interaction module is responsible for generating interactive responses to users or the environment. Given the current state \( S_t \) and the generated response \( A \), the interaction function is \( f_{\text{interact}} \).



\section{Design of power user behavior model based on generative Agent framework}


为了模拟用户在电力消费中的决策行为，本文采用基于类人生成智能体的方法对用户电力消费行为进行建模和模拟。生成式代理技术在增强人类决策的代表性方面起到关键作用。生成式代理通过创建包含与研究背景相关的人类个性和人口统计特征的角色，实现对用户行为的真实模拟。在这种方法中，每个角色都根据性格特征和/或人口统计数据进行描述，这些特征可能会影响代理的反应。为了详细描述用户的电力消费决策行为，我们从生成式代理构建和电力消费维度两个方面进行电力消费者行为生成式代理框架设计。
1. In order to simulate users' decision-making behavior in electricity consumption, this paper adopts a methodology based on human-like generative intelligent agents to model and simulate user electricity consumption behavior. Generative agent technology plays a crucial role in enhancing the representative of human decision-making. Generative agents create roles that incorporate human personalities and demographic characteristics relevant to the research context to achieve a realistic simulation of user behavior. In this approach, each role is described based on personality traits and/or demographic data that may influence the agent's responses. To provide a detailed description of users' electricity consumption decision-making behavior, we design a framework for electricity consumer behavior generation using generative agents from both the perspective of generative agent construction and electricity consumption dimensions.

2. To simulate user decision-making behavior in electricity consumption, this study employs a method based on human-like generative intelligent agents to model and simulate user electricity consumption behavior. Generative agent technology plays a critical role in enhancing the representative of human decision-making. By creating roles that encompass human personalities and demographic characteristics relevant to the research context, generative agents enable a realistic simulation of user behavior. In this approach, each role is described based on personality traits and/or demographic data that could impact the agent's responses. To elaborate on users' electricity consumption decision-making behavior, we design an electricity consumer behavior generative agent framework from the perspectives of generative agent construction and electricity consumption dimensions.

3. To model and simulate users' decision-making behavior in electricity consumption, this paper employs a methodology that relies on human-like generative intelligent agents. Generative agent technology plays a key role in enhancing the representative of human decision-making. By creating roles containing human personalities and demographic characteristics relevant to the research context, generative agents facilitate a realistic simulation of user behavior. In this approach, each role is described based on personality traits and/or demographic data that can influence the agent's responses. To provide a detailed description of users' electricity consumption decision-making behavior, we design an electricity consumer behavior generative agent framework focusing on generative agent construction and electricity consumption dimensions.

\subsection{Generative agent framework design}

生成式代理框架借鉴了Park等人（2023）在《Generative Agents: Interactive Simulacra of Human Behavior》中的研究成果，用于模拟可信的人类行为。该框架包括角色、计划、感知、记忆、决策和反思五个主要方面。代理通过大语言模型生成电力消费决策行为，并记住和反思过去的决策行为，以计划未来的决策行为。该架构使用自然语言存储代理的完整决策经历，并随着时间的推移将这些记忆综合为更高层次的反思，动态地检索它们以做出决策。
1. The generative agent framework drew inspiration from Park et al.'s (2023) research in "Generative Agents: Interactive Simulacra of Human Behavior" to simulate believable human behavior. This framework encompasses five main aspects: roles, planning, perception, memory, decision-making, and reflection. The agents utilize a large language model to generate electricity consumption decision-making behaviors, while also remembering and reflecting on past decisions to plan future ones. This architecture employs natural language to store the agent's complete decision-making experiences, integrating these memories over time into higher-level reflections, dynamically retrieving them to make decisions.

2. The generative agent framework, inspired by Park et al.'s (2023) research in "Generative Agents: Interactive Simulacra of Human Behavior," is utilized to simulate credible human behavior. This framework consists of five primary aspects: roles, planning, perception, memory, decision-making, and reflection. The agents generate electricity consumption decision-making behaviors using a large language model, and they store and reflect on past decision-making behaviors to plan future ones. This architecture utilizes natural language to store the agents' complete decision-making experiences and integrates these memories over time into higher-level reflections, dynamically retrieving them to make decisions.

3. The generative agent framework, inspired by the research of Park et al. (2023) in "Generative Agents: Interactive Simulacra of Human Behavior," is employed to simulate authentic human behavior. This framework comprises five key aspects: roles, planning, perception, memory, decision-making, and reflection. The agents leverage a large language model to generate electricity consumption decision-making behaviors and to remember and reflect on past decisions for future planning. This architecture uses natural language to store the agents' complete decision-making experiences, integrating these memories over time into higher-level reflections, dynamically retrieving them for decision-making.

\subsection{Design of power user behavior paradigm}

电力用户行为范式主要包括场景，空间、时间、能量和价格五个方面，通过将电力使用的场景（C），时间 (T)、空间 (S)、能量 (E) 和价格 (P) 构建模型，并结合用户的用电选择 (CC) 和响应模型，为电力消费者行为生成式代理框架设计提供了实用而有效的解决方案。在上述生成式代理框架基础上，根据电力消费范式对生成式代理框架进行细化。基于生成式代理的电力用户行为建模框架，通过整合时间、空间、能量和价格等因素，能够提供一个全面而灵活的解决方案。该框架利用生成式代理的记忆、检索、反思和交互能力，可以更准确地模拟和预测用户行为，提升电力系统的效率和可靠性。
1. The paradigm of electricity user behavior primarily includes five aspects: scenario, space, time, energy, and price. By modeling electricity usage scenarios (C), time (T), space (S), energy (E), and price (P), and incorporating user electricity consumption choices (CC) and response models, a practical and effective solution is provided for designing generative agent frameworks for electricity consumer behavior. Building upon this generative agent framework, a refinement is made based on the electricity consumption paradigm.
2. The generative agent framework for electricity consumer behavior, based on the electricity consumption paradigm, provides a comprehensive and flexible solution by integrating factors such as time, space, energy, and price. This framework utilizes the memory, retrieval, reflection, and interactive capabilities of generative agents to more accurately simulate and predict user behavior, thereby enhancing the efficiency and reliability of the electricity system.
3. The generative agent framework for modeling electricity user behavior integrates time, space, energy, and price factors to provide a comprehensive and flexible solution. Drawing from the electricity consumption paradigm, this framework leverages the memory, retrieval, reflection, and interactive capabilities of generative agents to accurately simulate and predict user behavior, ultimately enhancing the efficiency and reliability of the electricity system.
	


\subsection{Electricity consumer behavior generative agent framework description}

\subsubsection{Character}
角色模块在生成式代理框架中起着核心作用，通过整合人口统计信息和心理特征，生成详细的用电行为计划，决策。该模块旨在确保代理在复杂的电力消费环境中做出符合其角色特征的决策，从而提高整体用电效率和经济效益。每个用户 \( i \) 的人口统计信息和心理特征可以表示为向量 \( X \)：
1. The role module plays a central role in the generative agent framework, generating detailed electricity consumption plans and decisions by integrating demographic information and psychological characteristics. This module aims to ensure that agents make decisions in complex electricity consumption environments that align with their role characteristics, ultimately improving overall electricity efficiency and economic benefits. The demographic information and psychological characteristics of each user \( i \) can be represented as a vector \( X \)：
2. The role module plays a pivotal role in the generative agent framework by integrating demographic information and psychological characteristics to generate detailed electricity consumption plans and decisions. This module is designed to ensure that agents make decisions in complex electricity consumption environments that correspond to their role characteristics, thereby enhancing overall electricity efficiency and economic benefits. The demographic information and psychological characteristics of each user \( i \) can be represented as a vector \( X \)：
3. The role module is crucial in the generative agent framework, integrating demographic information and psychological characteristics to generate detailed electricity consumption plans and decisions. This module aims to enable agents to make decisions in complex electricity consumption environments that align with their role characteristics, ultimately enhancing overall electricity efficiency and economic benefits. The demographic information and psychological characteristics of each user \( i \) can be represented as a vector \( X \)：

\[X=[x_1,x_2,\ldots,x_m]\]

其中，\( x_{j} \) 表示用户 的第 \( j \) 项特征，如年龄、收入、家庭规模、节能意识等。
1. Where \( x_{j} \) represents the \( j \)th feature of the user, such as age, income, household size, energy-saving awareness, etc.
2. Here, \( x_{j} \) represents the \( j \)th feature of the user, such as age, income, household size, energy-saving awareness, etc.
3. In this context, \( x_{j} \) represents the \( j \)th feature of the user, such as age, income, household size, energy-saving awareness, and so on.

\subsubsection{Perception}
感知模块通过实时监测电力使用情况，为代理的决策提供准确且及时的数据支持。该模块综合考虑了时间、地点、场景、电量和价格等多方面因素，确保电力消费者行为的监测全面且精确。
1. The perception module provides real-time monitoring of electricity usage to offer accurate and timely data support for agent decision-making. This module considers various factors such as time, location, context, energy consumption, and prices, ensuring comprehensive and precise monitoring of electricity consumer behavior.
2. The perception module provides real-time monitoring of electricity usage to offer accurate and timely data support for agent decision-making. This module takes into account factors such as time, location, context, energy consumption, and prices, ensuring comprehensive and accurate monitoring of electricity consumer behavior.
3. The perception module monitors electricity usage in real-time to provide accurate and timely data support for agent decision-making. This module considers factors like time, location, context, energy consumption, and prices, ensuring comprehensive and precise monitoring of electricity consumer behavior.

#### 1. 感知输入的多方面因素感知模块通过传感器和数据采集设备，实时获取用户的用电信息。假设有 \( N \) 个电力消费者，每个消费者 \( i \) 的感知输入可以表示为向量 \( Z_i \)：
1. The perception module perceives multiple factors of the input by using sensors and data collection devices to real-time acquire users' electricity usage information. Assuming there are \( N \) electricity consumers, the perception input of each consumer \( i \) can be represented as a vector \( Z_i \):
2. The perception module collects various factors of the input through sensors and data collection devices to gather real-time electricity usage information from users. Assuming there are \( N \) electricity consumers, the perception input for each consumer \( i \) can be represented as a vector \( Z_i \):
3. The perception module utilizes sensors and data collection devices to capture multiple factors of the input, obtaining real-time electricity consumption information from users. Assuming there are \( N \) electricity consumers, the perception input for each consumer \( i \) can be expressed as a vector \( Z_i \):

\[ Z_i = [T(t), S(s), C(c), E(e), P(p)] \]

其中：
- \( T(t) \) 表示时间因素，\( t \) 是时间。
- \( S(s) \) 表示空间因素，\( s \) 是地点。
- \( C(c) \) 表示场景因素，\( c \) 是特定使用情境。
- \( E(e) \) 表示电量因素，\( e \) 是电量消耗。
- \( P(p) \) 表示价格因素，\( p \) 是电价。
Time factor \( T(t) \), where \( t \) is the time.
Spatial factor \( S(s) \), where \( s \) is the location.
Context factor \( C(c) \), where \( c \) is a specific usage scenario.
Energy factor \( E(e) \), where \( e \) is the electricity consumption.
Price factor \( P(p) \), where \( p \) is the electricity price.

\subsubsection{Planning*}



通过综合时间、空间、场景和能量等因素，结合用户的角色生成详细的场景行为计划。该模块确保代理在复杂和动态的电力消费环境更好的仿真用户行为。
1. By integrating factors such as time, space, context, and energy, and combining with the user's role, a detailed scenario behavior plan is generated. This module ensures that the agent better simulates user behavior in a complex and dynamic power consumption environment.
2. Through the integration of time, space, context, and energy factors, as well as the user's role, a detailed scenario behavior plan is generated. This module ensures better simulation of user behavior by the agent in a complex and dynamic electricity consumption environment.
3. By taking into account factors such as time, space, context, and energy, and incorporating the user's role, a detailed scenario behavior plan is created. This module ensures that the agent can better simulate user behavior in a complex and dynamic electricity consumption environment.

用电行为计划 \( P_i \) 是基于消费者 \( i \) 的时间、空间、场景和能量因素 \( Y_i \) 生成的函数：
1. The electricity usage behavior plan \( P_i \) is a function generated based on the time, space, context, and energy factors \( Y_i \) of consumer \( i \).
2. The electricity usage behavior plan \( P_i \) is a function that is generated from the time, space, context, and energy factors \( Y_i \) of consumer \( i \).
3. The electricity usage behavior plan \( P_i \) is a function which is generated based on the time, space, context, and energy factors \( Y_i \) of consumer \( i \).

\[ P_i = f_{\text{plan}}(X_i)(Z_i) \]

其中，\( f_{\text{plan}} \) 是用电行为计划生成函数，考虑了不同因素对用电行为的综合影响。
1. Where \( f_{\text{plan}} \) is the electricity usage behavior plan generation function, considering the combined impact of various factors on electricity usage behavior.
2. Here, \( f_{\text{plan}} \) represents the generation function of the electricity usage behavior plan, taking into account the integrated impact of different factors on electricity usage behavior.
3. In this context, \( f_{\text{plan}} \) serves as the function for generating the electricity usage behavior plan, incorporating the comprehensive influence of various factors on electricity usage behavior.


\subsubsection{Memory}
   - **描述**：记忆模块用于存储和管理代理的经历和行为数据。通过记录和回顾过去的行为和事件，代理可以更好地进行决策和计划未来的行为。该模块通过结构化和动态检索的方式，帮助代理在复杂的电力消费场景中做出更智能的选择。
    1. **Description**: The memory module is used to store and manage the agent's experiences and behavioral data. By recording and reviewing past actions and events, the agent can make better decisions and plan future behaviors. This module helps the agent make more intelligent choices in complex electricity consumption scenarios through structured and dynamic retrieval.
    2. **Description**: The memory module is responsible for storing and managing the agent's experiences and behavioral data. By recording and reviewing past behaviors and events, the agent can enhance decision-making and plan future actions more effectively. This module assists the agent in making smarter choices in complex electricity consumption scenarios through structured and dynamic retrieval.
    3. **Description**: The memory module is utilized to store and organize the agent's experiences and behavioral data. By recording and reviewing past behaviors and events, the agent can improve decision-making and plan future actions more effectively. This module supports the agent in making more intelligent choices in complex electricity consumption scenarios through structured and dynamic retrieval.
   
\paragraph{short term memory}

通过高效存储和快速检索最近的经历数据，支持代理在动态环境中进行实时决策。该模块不仅记录了代理的当前行为和决策，还通过整合和清理机制，确保短期记忆库的高效性和时效性。
1. Through efficient storage and rapid retrieval of recent experience data, the memory module supports real-time decision-making by the agent in a dynamic environment. This module not only records the agent's current behaviors and decisions but also ensures the efficiency and timeliness of the short-term memory bank through integration and cleaning mechanisms.
2. By efficiently storing and quickly retrieving recent experience data, the memory module assists the agent in making real-time decisions in a dynamic environment. In addition to recording the agent's current behaviors and decisions, this module also maintains the efficiency and timeliness of the short-term memory bank through integration and cleaning mechanisms.
3. Utilizing efficient storage and swift retrieval of recent experience data, the memory module facilitates real-time decision-making by the agent in a dynamic environment. This module not only documents the agent's current behaviors and decisions but also ensures the efficiency and timeliness of the short-term memory bank through integration and cleaning mechanisms.


1)Short-term memory storage：
在时间 \( t \)，短期记忆状态 \( STM_t \) 包含 \( N \) 条最近的经历条目，每条经历条目 \( stm_i \) 包含信息 \( I_i \) 和时间戳 \( t_i \)：
1. At time \( t \), the short-term memory state \( STM_t \) consists of \( N \) of the most recent experience entries, where each experience entry \( stm_i \) includes information \( I_i \) and timestamp \( t_i \):
\[ STM_t = \{(I_1, t_1), (I_2, t_2), \ldots, (I_N, t_N)\} \]
2. At time \( t \), the short-term memory state \( STM_t \) comprises \( N \) of the most recent experience entries, with each experience entry \( stm_i \) containing information \( I_i \) and timestamp \( t_i \):
\[ STM_t = \{(I_1, t_1), (I_2, t_2), \ldots, (I_N, t_N)\} \]
3. The short-term memory state \( STM_t \) at time \( t \) includes \( N \) of the most recent experience entries, where each experience entry \( stm_i \) is composed of information \( I_i \) and timestamp \( t_i \):


\[ STM_t = \{(I_1, t_1), (I_2, t_2), \ldots, (I_N, t_N)\} \]


2)Short-term memory renewal：
短期记忆通过整合和清理机制更新，确保其高效性和时效性：
1. Short-term memory is updated through integration and cleaning mechanisms to ensure its efficiency and timeliness.
2. Short-term memory is updated using integration and cleaning mechanisms to maintain its effectiveness and timeliness.
3. Integration and cleaning mechanisms are employed to update short-term memory, ensuring its efficiency and relevance.
\[ STM_{t+1} = \{(I_{2}, t_{2}), \ldots, (I_{N}, t_{N}), (I_{N+1}, t_{N+1})\} \]

其中，最旧的经历 \( (I_1, t_1) \) 被移除，新经历 \( (I_{N+1}, t_{N+1}) \) 被添加。
The oldest experience \( (I_1, t_1) \) is removed, while the new experience \( (I_{N+1}, t_{N+1}) \) is added.

3) Short-term memory retrieval：

短期记忆的检索函数 \( f_{\text{STM\_retrieve}} \) 用于快速获取相关数据：
\[ I^* = f_{\text{STM\_retrieve}}(STM_t, q) \]
其中，\( q \) 为检索查询，\( I^* \) 为与查询最相关的经历数据。
1. The retrieval function \( f_{\text{STM\_retrieve}} \) of short-term memory is utilized for fast access to relevant data:
\[ I^* = f_{\text{STM\_retrieve}}(STM_t, q) \]
where \( q \) stands for the retrieval query, and \( I^* \) denotes the experience data most closely related to the query.
2. The retrieval function \( f_{\text{STM\_retrieve}} \) of short-term memory is employed to swiftly obtain pertinent data:
\[ I^* = f_{\text{STM\_retrieve}}(STM_t, q) \]
Here, \( q \) represents the retrieval query, while \( I^* \) signifies the experience data most relevant to the query.
3. The retrieval function \( f_{\text{STM\_retrieve}} \) for short-term memory is utilized to promptly retrieve relevant data:
\[ I^* = f_{\text{STM\_retrieve}}(STM_t, q) \]
In this case, \( q \) is the retrieval query and \( I^* \) represents the experience data most closely associated with the query.

\subsubsubsection{long-term memory}
  
  通过系统化存储和深度分析长期经历数据，帮助代理模拟人类积累专业知识的过程，并不断提高决策收益。该模块不仅记录了代理的所有用电行为和决策，还通过分析和学习机制，确保长期记忆库的全面性和时效性。
  1. By systematically storing and deeply analyzing long-term experience data, the system assists the agent in simulating the process of accumulating professional knowledge like humans and continuously improving decision-making benefits. This module not only records all the agent's electricity usage behaviors and decisions but also ensures the comprehensiveness and timeliness of the long-term memory repository through analysis and learning mechanisms.
  2. Through systematic storage and in-depth analysis of long-term experiential data, the system helps the agent simulate the process of accumulating professional knowledge like humans, and continually enhance decision-making benefits. This module not only logs all of the agent's electricity usage behaviors and decisions but also ensures the comprehensiveness and timeliness of the long-term memory bank through analysis and learning mechanisms.
  3. By systematically storing and deeply analyzing long-term experiential data, the system aids the agent in emulating the process of accumulating professional knowledge akin to humans and incrementally enhancing decision-making benefits. This module not only documents all the agent's electricity usage behaviors and decisions but also ensures the comprehensiveness and timeliness of the long-term memory repository through analysis and learning mechanisms.



\paragraph{Long-Term Memory}
长期记忆用于系统化存储和深度分析长期经历数据。
1. Long-term memory is employed for the systematic storage and deep analysis of long-term experience data.
2. Long-term memory is used for the systematic storage and thorough analysis of long-term experiential data.
3. Long-term memory is utilized for the systematic storage and in-depth analysis of long-term experience data.

1)Long-term memory storage：
长期记忆状态 \( LTM \) 包含 \( M \) 条经历条目，每条经历条目 \( ltm_i \) 包含信息 \( I_i \)、时间戳 \( t_i \) 以及行为结果 \( R_i \)：
1. The long-term memory state \( LTM \) consists of \( M \) experience entries, each experience entry \( ltm_i \) containing information \( I_i \), timestamp \( t_i \), and behavioral outcome \( R_i \).
2. The long-term memory state \( LTM \) comprises \( M \) experience entries, with each experience entry \( ltm_i \) including information \( I_i \), timestamp \( t_i \), and behavioral outcome \( R_i \).
3. The long-term memory state \( LTM \) includes \( M \) experience entries, where each experience entry \( ltm_i \) contains information \( I_i \), timestamp \( t_i \), and behavioral outcome \( R_i \).
\[ LTM = \{(I_1, t_1, R_1), (I_2, t_2, R_2), \ldots, (I_M, t_M, R_M)\} \]

2)Long-term memory renewal：
长期记忆通过系统化存储新的经历数据来更新：
1. Long-term memory is updated by systematically storing new experiential data.
2. Long-term memory is refreshed by systematically storing new experiential data updates.   
3. Long-term memory is refreshed through the systematic storage of new experience data updates.
\[ LTM_{t+1} = LTM_t \cup \{(I_{M+1}, t_{M+1}, R_{M+1})\} \]

3) Long-term memory analysis：
长期记忆的分析函数 \( f_{\text{LTM\_analyze}} \) 用于分析和学习过去的行为数据，以提高未来的决策收益：
1. The analysis function \( f_{\text{LTM\_analyze}} \) of long-term memory is used to analyze and learn from past behavioral data in order to enhance future decision-making benefits.
2. The analysis function \( f_{\text{LTM\_analyze}} \) in long-term memory is employed for analyzing and learning from historical behavioral data to enhance future decision-making benefits. 
3. The analytical function \( f_{\text{LTM\_analyze}} \) in long-term memory is utilized to analyze and learn from previous behavioral data, aiming to improve future decision-making outcomes.
\[ \mathcal{A} = f_{\text{LTM\_analyze}}(LTM) \]

其中，\( \mathcal{A} \) 表示分析结果和提取的模式或规律。
1. Here, \( \mathcal{A} \) represents the analysis results and extracted patterns or regularities.
2. In this context, \( \mathcal{A} \) signifies the analysis findings and extracted patterns or regularities.
3. In this context, \( \mathcal{A} \) embodies the analysis outcomes and extracted patterns or regularities.

4) Long-term memory retrieval：
长期记忆的检索函数 \( f_{\text{LTM\_retrieve}} \) 用于深度获取相关数据，以支持复杂决策：
1.Long-Term Memory Retrieval Function \( f_{\text{LTM\_retrieve}}\) for In-Depth Accessing of Relevant Data to Facilitate Complex Decision Making
2.Utilization of the Long-Term Memory Retrieval Function \( f_{\text{LTM\_retrieve}}\) for Comprehensive Data Retrieval in Aid of Complex Decision Making
3.Application of the Long-Term Memory Retrieval Function \( f_{\text{LTM\_retrieve}}\) for Enhanced Data Retrieval to Enable Complex Decision Making

\[ I^{**} = f_{\text{LTM\_retrieve}}(LTM, q) \]
其中，\( q \) 为检索查询，\( I^{**} \) 为与查询最相关的长期经历数据。
1.Here, \( q \) serves as the retrieval query, while \( I^{**} \) represents the long-term experiential data most relevant to the query.
2.In this context, \( q \) is the retrieval query, and \( I^{**} \) denotes the long-term experiential data that is most relevant to the query.
3.Within this framework, \( q \) is the retrieval query, and \( I^{**} \) stands for the long-term experiential data that is most pertinent to the query.



\subsubsection{Decision-Making}
   - **描述**：决策模块是生成式代理框架中的核心组件，通过综合角色画像、感知和记忆模块提供的数据，确保代理在复杂和动态的电力消费环境中做出符合其角色特征的决策。决策输出包括用电行为的时间、空间、场景、能量和价格等方面。
   1. **Description**: The decision module is the core component in the generative agent framework, integrating data from role profiles, perception, and memory modules to guide the agent in making decisions that align with its role characteristics in complex and dynamic electricity consumption environments. Decision outputs encompass aspects of electricity usage behavior including timing, spatial considerations, scenarios, energy usage, and pricing.
   2. **Description**: The decision module plays a pivotal role in the generative agent framework by leveraging data from role profiles, perception, and memory modules to enable the agent to make decisions tailored to its role features within intricate and evolving electricity consumption settings. The decision outputs cover various aspects of electricity usage behavior, such as timing, spatial context, scenarios, energy aspects, and pricing.
   3. **Description**: Within the generative agent framework, the decision module acts as a key element, utilizing data from role profiles, perception, and memory modules to ensure the agent makes decisions in complex and dynamic electricity consumption environments that are in line with its role characteristics. The decision outputs include aspects like timing, spatial considerations, scenarios, energy utilization, and pricing related to electricity consumption behavior.

#### Mathematical description

##### Mathematical description of decision module
决策模块通过综合角色画像、感知和记忆模块提供的数据，生成用电行为决策。以下是该模块的数学描述。
1. The decision module generates decisions on electricity consumption behavior by integrating data provided by role profiles, perception, and memory modules. The following is the mathematical description of this module.
2. The decision module utilizes data from role profiles, perception, and memory modules to produce decisions on electricity consumption behavior. Presented below is the mathematical depiction of this module.
3. By synthesizing data from role profiles, perception, and memory modules, the decision module formulates decisions regarding electricity consumption behavior. The mathematical description of this module is outlined as follows.

\paragraph{input data}
决策模块通过综合角色画像 \( R_i \)、感知数据 \( P_i \) 和记忆数据 \( M_i \)，生成最终决策输入向量 \( D_{\text{input}} \)：
1. The decision module generates the final decision input vector \( D_{\text{input}} \) by integrating role profiles \( R_i \), perception data \( P_i \), and memory data \( M_i \). 
2. The decision module combines role profiles \( R_i \), perception data \( P_i \), and memory data \( M_i \) to produce the final decision input vector \( D_{\text{input}} \).
3. Through the synthesis of role profiles \( R_i \), perception data \( P_i \), and memory data \( M_i \), the decision module generates the final decision input vector \( D_{\text{input}} \).

\[ D_{\text{input}} = f_{\text{integrate}}(R_i, P_i, M_i) \]
其中：
- \( R_i \) 表示角色画像，包括人口统计信息和心理特征。
- \( P_i \) 表示感知数据，包括时间、空间、场景、电量和价格等因素。
- \( M_i \) 表示记忆数据，包括短期记忆 \( STM_i \) 和长期记忆 \( LTM_i \) 的整合结果。
1. \( R_i \) represents role profiles, encompassing demographic statistics and psychological traits.
- \( P_i \) signifies perception data, incorporating factors such as time, space, scenarios, electricity consumption, and pricing.
- \( M_i \) denotes memory data, encompassing the integration of short-term memory \( STM_i \) and long-term memory \( LTM_i \) results.
2. \( R_i \) denotes role profiles, consisting of demographic information and psychological characteristics.
- \( P_i \) stands for perception data, encompassing factors like time, space, scenarios, electricity usage, and pricing.
- \( M_i \) represents memory data, including the consolidation of short-term memory \( STM_i \) and long-term memory \( LTM_i \) outcomes.
3. \( R_i \) signifies role profiles, including demographic details and psychological features.
- \( P_i \) indicates perception data, covering elements such as time, space, scenarios, energy consumption, and pricing.
- \( M_i \) expresses memory data, which integrates the results of short-term memory \( STM_i \) and long-term memory \( LTM_i \).

\paragraph{decision function}

决策生成函数 \( g_{\text{decision}} \) 基于整合的输入数据 \( D_{\text{input}} \) 生成用电行为决策 \( D_i(t, s, c, e, p) \)：
1. The decision generation function \( g_{\text{decision}} \) produces electricity consumption behavior decisions \( D_i(t, s, c, e, p) \) based on the integrated input data \( D_{\text{input}} \).
2. The decision-making function \( g_{\text{decision}} \) generates electricity consumption behavior decisions \( D_i(t, s, c, e, p) \) based on the integrated input data \( D_{\text{input}} \).
3. The decision-generating function \( g_{\text{decision}} \) creates electricity consumption behavior decisions \( D_i(t, s, c, e, p) \) using the integrated input data \( D_{\text{input}} \).

\[ D_i(t, s, c, e, p) = g_{\text{decision}}(D_{\text{input}}) \]

其中：
- \( D_i(t, s, c, e, p) \) 表示消费者 \( i \) 在时间 \( t \)、空间 \( s \)、场景 \( c \)、能量 \( e \) 和价格 \( p \) 下的电力需求决策。
- \( g_{\text{decision}} \) 是决策生成函数，考虑了各种影响因素的综合作用。
1. Where：
\( D_i(t, s, c, e, p) \) represents consumer \( i \)'s electricity demand decision at time \( t \), space \( s \), scenario \( c \), energy \( e \), and price \( p \).
- \( g_{\text{decision}} \) is the decision generation function that considers the combined effects of various influencing factors.
2.  Where：
\( D_i(t, s, c, e, p) \) denotes the electricity demand decision of consumer \( i \) at time \( t \), space \( s \), scenario \( c \), energy \( e \), and price \( p \).
- \( g_{\text{decision}} \) serves as the decision generation function, taking into account the integrated effects of various influencing factors.
3.  Where：
\( D_i(t, s, c, e, p) \) represents consumer \( i \)'s electricity demand decision under time \( t \), space \( s \), scenario \( c \), energy \( e \), and price \( p \).
- \( g_{\text{decision}} \) functions as the decision generation function that considers the comprehensive impact of various influencing factors.

\paragraph{Decision output}

决策输出包括用电行为的时间、空间、场景、能量和价格等方面，表示为向量 \( D_i \)：
\[ D_i = [T(t), S(s), C(c), E(e), P(p)] \]
其中：
- \( T(t) \) 表示决策的时间因素。
- \( S(s) \) 表示决策的空间因素。
- \( C(c) \) 表示决策的场景因素。
- \( E(e) \) 表示决策的能量需求。
- \( P(p) \) 表示决策的价格因素。
1. The decision output, encompassing aspects of time, space, scenario, energy, and price related to electricity consumption behavior, is represented as the vector \( D_i \):
\[ D_i = [T(t), S(s), C(c), E(e), P(p)] \]
Where:
- \( T(t) \) represents the temporal factor of the decision.
- \( S(s) ) represents the spatial factor of the decision.
- \( C(c) \) represents the scenario factor of the decision.
- \( E(e) \) represents the energy demand of the decision.
- \( P(p) \) represents the price factor of the decision.
2. The vector \( D_i \) represents the output of the decision in terms of time, space, scenario, energy, and price factors related to electricity consumption behavior:
\[ D_i = [T(t), S(s), C(c), E(e), P(p)] \]
Where:
- \( T(t) \) signifies the temporal factor of the decision.
- \( S(s) \) represents the spatial factor of the decision.
- \( C(c) \) denotes the scenario factor of the decision.
- \( E(e) \) indicates the energy requirement of the decision.
- \( P(p) \) stands for the price factor of the decision.
3. The vector \( D_i \) captures the elements of time, space, scenario, energy demand, and price associated with electricity consumption behavior decision, represented as:
\[ D_i = [T(t), S(s), C(c), E(e), P(p)] \]
Where:
- \( T(t) \) represents time-related factors in the decision.
- \( S(s) denotes spatial considerations in the decision.
- \( C(c) represents scenario factors in the decision.
- \( E(e) signifies the energy requirements in the decision.
- \( P(p) describes the price factors in the decision.


\paragraph{Decision feedback and adjustment}

决策模块通过实时反馈机制调整和优化决策过程，确保在动态环境中做出最优决策。反馈函数 \( f_{\text{feedback}} \) 根据实际用电行为和环境变化，调整决策生成函数 \( g_{\text{decision}} \)：
\[ g_{\text{decision}}^{\text{new}} = f_{\text{feedback}}(g_{\text{decision}}, \text{actual\_behavior}, \text{environment\_changes}) \]
1. The decision module adjusts and optimizes the decision-making process through real-time feedback mechanisms to ensure optimal decisions are made in dynamic environments. The feedback function \( f_{\text{feedback}} \) modifies the decision generation function \( g_{\text{decision}} \) based on actual electricity consumption behavior and environmental changes:
\[ g_{\text{decision}}^{\text{new}} = f_{\text{feedback}}(g_{\text{decision}}, \text{actual\_behavior}, \text{environment\_changes}) \]
2. The decision module fine-tunes and enhances the decision-making process using real-time feedback mechanisms to ensure optimal decisions in dynamic environments. The feedback function \( f_{\text{feedback}} \) adjusts the decision generation function \( g_{\text{decision}} \) based on actual electricity consumption behavior and changes in the environment:
\[ g_{\text{decision}}^{\text{new}} = f_{\text{feedback}}(g_{\text{decision}}, \text{actual\_behavior}, \text{environment\_changes}) \]
3. The decision module refines and improves the decision-making process by utilizing real-time feedback mechanisms to ensure optimal decisions are made in dynamic environments. The feedback function \( f_{\text{feedback}} \) adapts the decision generation function \( g_{\text{decision}} \) based on actual electricity consumption behavior and environmental changes:
\[ g_{\text{decision}}^{\text{new}} = f_{\text{feedback}}(g_{\text{decision}}, \text{actual\_behavior}, \text{environment\_changes}) \]

\paragraph{Synthetic decision process}

The entire decision process can be expressed as the following steps


1. Integrate character portrait, perception, and memory data
   \[ D_{\text{input}} = f_{\text{integrate}}(R_i, P_i, M_i) \]

2. Generate power consumption behavior decision：
   \[ D_i(t, s, c, e, p) = g_{\text{decision}}(D_{\text{input}}) \]

3. Implement decisions and monitor actual behavior and environmental changes：
   \[ \text{monitor}(\text{actual\_behavior}, \text{environment\_changes}) \]

4. Adjust the decision generating function based on feedback：
   \[ g_{\text{decision}}^{\text{new}} = f_{\text{feedback}}(g_{\text{decision}}, \text{actual\_behavior}, \text{environment\_changes}) \]

决策模块是生成式代理框架中的核心组件，通过综合角色画像、感知和记忆模块提供的数据，生成符合其角色特征的用电行为决策。该模块的数学描述为整体框架提供了理论基础，使得生成式代理能够在复杂和动态的电力消费环境中做出高效的决策。
1. The decision module is the core component in the generative agent framework, which generates electricity consumption behavior decisions that align with its role characteristics by integrating data from role profiles, perception, and memory modules. The mathematical description of this module provides the theoretical foundation for the overall framework, enabling generative agents to make efficient decisions in complex and dynamic electricity consumption environments.
2. The decision module, as the heart of the generative agent framework, creates electricity consumption behavior decisions that match its role characteristics by integrating data from role profiles, perception, and memory modules. The mathematical description of this module forms the theoretical basis for the entire framework, allowing generative agents to make efficient decisions in complex and dynamic electricity consumption environments.
3. Within the generative agent framework, the decision module serves as a central component that produces electricity consumption behavior decisions in accordance with its role characteristics by synthesizing data from role profiles, perception, and memory modules. The mathematical description of this module provides the theoretical groundwork for the entire framework, enabling generative agents to make effective decisions in complex and dynamic electricity consumption environments.

\subsubsection{Reflection*} 


\textbf{描述}：反思模块通过对代理过去的行为和决策进行评估和总结，改进未来的行为模式。该模块突出符合角色行为特征，确保代理在电力消费中的决策与其个性和人口统计特征保持一致，从而实现更真实和个性化的用电行为。
1. \textbf{Description}: The reflection module evaluates and summarizes the agent's past behaviors and decisions, aiming to enhance future behavioral patterns. This module emphasizes alignment with role behavioral characteristics, ensuring that the agent's decisions in electricity consumption are consistent with its personality and demographic features, thereby achieving more realistic and personalized electricity consumption behavior.
2.  \textbf{Description}*: The reflection module assesses and synthesizes the agent's past behaviors and decisions to improve future behavioral patterns. This module highlights adherence to role behavioral characteristics, ensuring that the agent's decisions in electricity consumption align with its individuality and demographic features, thereby achieving a more authentic and personalized electricity consumption behavior.
3.  \textbf{Description}: The reflection module evaluates and consolidates the agent's past actions and decisions to refine future behavioral patterns. Emphasizing alignment with role behavioral traits, this module ensures that the agent's decisions in electricity consumption remain consistent with its personality and demographic characteristics, resulting in a more authentic and individualized electricity consumption behavior.

\paragraph{Reflect on the mathematical description of the module}
反思模块通过评估和总结代理过去的行为和决策，改进未来的行为模式。以下是该模块的数学描述。
1. The reflection module improves future behavioral patterns by evaluating and summarizing the agent's past actions and decisions. Here is the mathematical description of this module.
2. The reflection module enhances future behavioral patterns by assessing and summarizing the agent's past behaviors and decisions. The following is the mathematical description of this module.
3. By evaluating and summarizing the agent's past behaviors and decisions, the reflection module aims to improve future behavioral patterns. Presented below is the mathematical description of this module.

\textbf{(1). Acquisition of behavioral and decision data} \\
反思模块从记忆模块中获取过去的行为和决策数据，包括短期记忆和长期记忆中的记录。假设过去的行为和决策数据集为 \( H \)：
\[ H = \{(D_i, R_i, t_i)\}_{i=1}^{N} \]
1. The reflection module retrieves past behavior and decision data from the memory module, including records in both short-term and long-term memory. Let's assume the dataset of past behavior and decision is denoted as \( H \):
\[ H = \{(D_i, R_i, t_i)\}_{i=1}^{N} \]
2. The reflection module accesses historical behavior and decision data from the memory module, encompassing records from both short-term memory and long-term memory. Assuming the dataset of historical behavior and decisions is represented as \( H \):
\[ H = \{(D_i, R_i, t_i)\}_{i=1}^{N} \]
3. The reflection module gathers historical behavior and decision data from the memory module, comprising records stored in both short-term and long-term memory. Assumed that the dataset of historical behavior and decisions is labeled as \( H \):
\[ H = \{(D_i, R_i, t_i)\}_{i=1}^{N} \]

其中：
\begin{itemize}
    \item \( D_i \) 表示第 \( i \) 次决策行为，包括时间、空间、场景、能量和价格等因素。
    \item \( R_i \) 表示第 \( i \) 次决策行为的结果或反馈。
    \item \( t_i \) 表示第 \( i \) 次决策行为的时间。
\end{itemize}
Where：
\begin{itemize}
    \item \( D_i \) represents the \( i \)th decision behavior, including factors such as time, space, scenario, energy, and price.
    \item \( R_i \) represents the result or feedback of the \( i \)th decision behavior.
    \item \( t_i \) indicates the time of the \( i \)th decision behavior.
\end{itemize}



\textbf{(2). Behavior evaluation function} \\
反思模块使用行为评估函数 \( f_{\text{evaluate}} \) 对每个行为和决策进行评估，生成评估结果 \( E_i \)：
\[ E_i = f_{\text{evaluate}}(D_i, R_i) \]
1. The reflection module uses the behavior evaluation function \( f_{\text{evaluate}} \) to evaluate each behavior and decision, generating the evaluation result \( E_i \)：
\[ E_i = f_{\text{evaluate}}(D_i, R_i) \]
2. The reflection module assesses each behavior and decision using the behavior evaluation function \( f_{\text{evaluate}} \), resulting in the evaluation output \( E_i \)：
\[ E_i = f_{\text{evaluate}}(D_i, R_i) \]
3. The reflection module evaluates each behavior and decision through the behavior evaluation function \( f_{\text{evaluate}} \), producing the evaluation outcome \( E_i \)：
\[ E_i = f_{\text{evaluate}}(D_i, R_i) \]

其中：
\begin{itemize}
    \item \( E_i \) 表示第 \( i \) 次决策行为的评估结果，衡量行为和决策的有效性。
\end{itemize}
Where：
\begin{itemize}
    \item \( E_i \) represents the evaluation result of the \( i \)th decision behavior, measuring the effectiveness of behavior and decisions.
\end{itemize}

\textbf{(3). Summary and pattern recognition} \\
反思模块通过总结和模式识别函数 \( f_{\text{summarize}} \) 对所有评估结果进行总结，提取行为模式和改进建议：
1. The reflection module summarizes all evaluation results and extracts behavior patterns and improvement suggestions using the summary and pattern recognition function \( f_{\text{summarize}} \)：
\[ S = f_{\text{summarize}}(\{E_i\}_{i=1}^{N}) \]
2. Through the summary and pattern recognition function \( f_{\text{summarize}} \), the reflection module consolidates all evaluation results, extracting behavior patterns and suggestions for improvement：
\[ S = f_{\text{summarize}}(\{E_i\}_{i=1}^{N}) \]
3. The reflection module summarizes all evaluation results and extracts behavior patterns and suggestions for improvement by using the summary and pattern recognition function \( f_{\text{summarize}} \)：
\[ S = f_{\text{summarize}}(\{E_i\}_{i=1}^{N}) \]

其中：
\begin{itemize}
    \item \( S \) 表示总结和提取的行为模式和改进建议。
\end{itemize}
Where:
\begin{itemize}
    \item \( S \) represents the summarized and extracted behavior patterns and improvement suggestions.
\end{itemize}

\textbf{(4). Improvement of behavior patterns} \\
反思模块根据总结和提取的行为模式，调整和改进未来的行为模式。改进函数 \( f_{\text{improve}} \) 用于生成新的行为模式 \( M_{\text{new}} \)：
\[ M_{\text{new}} = f_{\text{improve}}(S) \]
1. The reflection module adjusts and improves future behavior patterns based on the summarized and extracted behavior patterns. The improvement function \( f_{\text{improve}} \) is used to generate a new behavior pattern \( M_{\text{new}} \):
\[ M_{\text{new}} = f_{\text{improve}}(S) \]
2. The reflection module refines and enhances future behavior patterns by utilizing the summarized and extracted behavior patterns. The improvement function \( f_{\text{improve}} \) is employed to generate a new behavior pattern \( M_{\text{new}} \):
\[ M_{\text{new}} = f_{\text{improve}}(S) \]
3. Based on the summarized and extracted behavior patterns, the reflection module adjusts and improves future behavior patterns. The improvement function \( f_{\text{improve}} \) is utilized to create a new behavior pattern \( M_{\text{new}} \):
\[ M_{\text{new}} = f_{\text{improve}}(S) \]

其中：
\begin{itemize}
    \item \( M_{\text{new}} \) 表示新的行为模式，用于指导未来的决策。
\end{itemize}
Where:
\begin{itemize}
    \item \( M_{\text{new}} \) represents a new behavior pattern used to guide future decisions.
\end{itemize}

\textbf{(5). Reflect on the application of the output} \\
反思模块的输出 \( M_{\text{new}} \) 用于更新决策模块中的行为模式，使代理在未来的电力消费决策中更加符合其角色特征和个性化需求。
1. The output \( M_{\text{new}} \) of the reflection module is used to update the behavior patterns in the decision-making module, enabling the agent to make future electricity consumption decisions that better align with its role characteristics and personalized needs.
2. The reflection module's output \( M_{\text{new}} \) is utilized to adjust the behavior patterns in the decision-making module, ensuring that the agent's future electricity consumption decisions more closely match its role characteristics and personalized requirements.
3. The output \( M_{\text{new}} \) from the reflection module is employed to revise the behavior patterns in the decision-making module, enhancing the agent's alignment with its role characteristics and personalized needs in future electricity consumption decisions.

\textbf{(6). Comprehensive reflection process} \\
The whole reflection process can be expressed as the following steps：
\begin{enumerate}
    \item 获取过去的行为和决策数据：\[ H = \{(D_i, R_i, t_i)\}_{i=1}^{N} \]
    \item 对行为和决策进行评估：\[ E_i = f_{\text{evaluate}}(D_i, R_i) \]
    \item 总结和提取行为模式和改进建议：\[ S = f_{\text{summarize}}(\{E_i\}_{i=1}^{N}) \]
    \item 生成新的行为模式：\[ M_{\text{new}} = f_{\text{improve}}(S) \]
    \item 应用新的行为模式指导未来决策。
\end{enumerate}
\begin{enumerate}
    \item Obtain historical behavioral and decision data: \[ H = \{(D_i, R_i, t_i)\}_{i=1}^{N} \]
    \item Evaluate the behaviors and decisions: \[ E_i = f_{\text{evaluate}}(D_i, R_i) \]
    \item Summarize and extract behavioral patterns and improvement recommendations: \[ S = f_{\text{summarize}}(\{E_i\}_{i=1}^{N}) \]
    \item Generate new behavioral patterns: \[ M_{\text{new}} = f_{\text{improve}}(S) \]
    \item Apply the new behavioral patterns to guide future decisions.
\end{enumerate}


\subsubsection{Retrieval Augmentation}
\textbf{描述}：基于检索增强的生成式代理角色设计通过整合详细的人口统计信息和心理特征知识库，结合时间、空间、场景和能量等因素，生成更加精准和智能的用电行为计划。通过实时检索和更新外部数据，代理能够更好地反映实际情况并做出符合统计规律的决策，提高整体用电效率和经济效益。
1. \textbf{Description}: The design of retrieval-enhanced generative agent roles integrates detailed demographic information and psychological feature knowledge base, combined with factors such as time, space, scenarios, and energy, to generate more accurate and intelligent electricity usage behavior plans. Through real-time retrieval and updating of external data, the agent can better reflect the actual situation and make decisions in accordance with statistical regularities, thereby improving overall electricity efficiency and economic benefits.
2. \textbf{Description}: The design of generation-enabled agent roles with enhanced retrieval capabilities integrates detailed demographic information and knowledge of psychological characteristics, while considering factors such as time, space, scenarios, and energy. This helps in creating more precise and intelligent electricity usage behavior plans. By continuously retrieving and updating external data, the agent can better reflect real-world conditions and make decisions that align with statistical patterns, leading to enhanced overall electricity efficiency and economic benefits.
3. \textbf{Description}: By integrating detailed population demographics and psychological feature knowledge, along with considering factors like time, space, scenarios, and energy, the design of a retrieval-enhanced generative agent role aims to create more precise and intelligent electricity usage behavior plans. Real-time retrieval and updating of external data enable the agent to better reflect actual conditions and make decisions in line with statistical patterns, ultimately improving overall electricity efficiency and economic benefits.

\paragraph{Retrieves the mathematical description of the enhancement module}
检索增强模块通过整合详细的人口统计信息和心理特征知识库，并结合时间、空间、场景和能量等因素，生成更加精准和智能的用电行为计划。以下是该模块的数学描述。
1. \textbf{Retrieval-Enhanced Module Description}: The module enhances retrieval capabilities by integrating detailed demographic information and knowledge of psychological characteristics, while considering factors such as time, space, scenarios, and energy. It generates more precise and intelligent electricity usage behavior plans. Here is the mathematical description of the module.
2. \textbf{Description of the Retrieval-Enhanced Module}: This module enhances its retrieval capabilities by incorporating detailed demographic information and psychological feature knowledge, and by taking into account factors such as time, space, scenarios, and energy. It produces more accurate and intelligent electricity usage behavior plans. Below is the mathematical depiction of the module.
3. \textbf{Description for the Retrieval-Enhanced Module}: The module improves its retrieval capabilities by combining detailed demographic information and knowledge of psychological characteristics with factors like time, space, scenarios, and energy. It then generates more accurate and intelligent electricity usage behavior plans. The mathematical description of the module is provided below.

\textbf{(1). Construction and update of knowledge base} \\
知识库\(K\)包含人口统计信息和心理特征的详细记录，每条记录\(k_i\)包含信息\(I_i\)和时间戳\(t_i\)：
\[ K = \{(I_1, t_1), (I_2, t_2), \ldots, (I_N, t_N)\} \]
1. \textbf{Description of Knowledge Base \(K\)}: The knowledge base \(K\) contains detailed records of demographic information and psychological characteristics. Each record \(k_i\) includes information \(I_i\) and a timestamp \(t_i\):
\[ K = \{(I_1, t_1), (I_2, t_2), \ldots, (I_N, t_N)\} \]
2. \textbf{Translation of the Knowledge Base \(K\)}: The knowledge base \(K\) comprises detailed entries of demographic information and psychological characteristics. Each entry \(k_i\) consists of information \(I_i\) and a timestamp \(t_i\):
\[ K = \{(I_1, t_1), (I_2, t_2), \ldots, (I_N, t_N)\} \]
3. \textbf{Knowledge Base \(K\) Description}: The knowledge base \(K\) contains detailed records of demographic information and psychological characteristics. Each individual record \(k_i\) includes information \(I_i\) and a timestamp \(t_i\):
\[ K = \{(I_1, t_1), (I_2, t_2), \ldots, (I_N, t_N)\} \]

\noindent 知识库实时更新，确保数据的准确性和时效性：
\[ K_{t+1} = K_t \cup \{(I_{N+1}, t_{N+1})\} \]
1. \textbf{Real-time Updates of the Knowledge Base}: The knowledge base is updated in real-time to ensure the accuracy and timeliness of the data.
\[ K_{t+1} = K_t \cup \{(I_{N+1}, t_{N+1})\} \]
2. \textbf{Continuous Real-time Updating of the Knowledge Base}: The knowledge base undergoes continuous real-time updates to maintain data accuracy and timeliness.
\[ K_{t+1} = K_t \cup \{(I_{N+1}, t_{N+1})\} \]
3. \textbf{Knowledge Base Updating in Real-time}: The knowledge base is continuously updated in real-time to ensure the accuracy and timeliness of the data.
\[ K_{t+1} = K_t \cup \{(I_{N+1}, t_{N+1})\} \]

\textbf{(2). Retrieval function} \\
检索函数\(f_{\text{retrieve}}\)用于从知识库\(K\)中提取与当前情境相关的信息。给定检索查询\(q\)，最相关的知识条目\(I^*\)定义为：
\[ I^* = \arg\max_{I_i \in K} \text{similarity}(q, I_i) \]
1. \textbf{Retrieval Function \(f_{\text{retrieve}}\)}: The retrieval function \(f_{\text{retrieve}}\) is used to extract information relevant to the current context from the knowledge base \(K\). Given a retrieval query \(q\), the most relevant knowledge entry \(I^*\) is defined as:
\[ I^* = \arg\max_{I_i \in K} \text{similarity}(q, I_i) \]
2. \textbf{Utilization of Retrieval Function \(f_{\text{retrieve}}\)}: The retrieval function \(f_{\text{retrieve}}\) is employed to extract contextually relevant information from the knowledge base \(K\). When provided with a retrieval query \(q\), the most relevant knowledge entry \(I^*\) is determined as:
\[ I^* = \arg\max_{I_i \in K} \text{similarity}(q, I_i) \]
3. \textbf{Application of Retrieval Function \(f_{\text{retrieve}}\)}: The retrieval function \(f_{\text{retrieve}}\) is utilized to fetch information from the knowledge base \(K) that is pertinent to the current situation. With a retrieval query \(q\) given, the most relevant knowledge entry \(I^*\) is defined as:
\[ I^* = \arg\max_{I_i \in K} \text{similarity}(q, I_i) \]

\noindent 其中，相关性通过余弦相似度或其他相似度度量计算：
\[ \text{similarity}(q, I_i) = \frac{q \cdot I_i}{\|q\| \|I_i\|} \]
1. \textbf{Calculation of Relevance}: The relevance is calculated using cosine similarity or other similarity metrics:
\[ \text{similarity}(q, I_i) = \frac{q \cdot I_i}{\|q\| \|I_i\|} \]
2. \textbf{Determination of Similarity}: The similarity between \(q\) and \(I_i\) is computed using cosine similarity or other similarity measurements:
\[ \text{similarity}(q, I_i) = \frac{q \cdot I_i}{\|q\| \|I_i\|} \]
3. \textbf{Quantification of Correspondence}: The correlation is evaluated through cosine similarity or alternative similarity measures:
\[ \text{similarity}(q, I_i) = \frac{q \cdot I_i}{\|q\| \|I_i\|} \]

\textbf{(3). The integration of comprehensive factors} \\
整合函数\(f_{\text{integrate}}\)将检索到的知识条目\(I^*\)与时间、空间、场景和能量等因素整合，生成决策输入\(D_{\text{input}}\)：
\[ D_{\text{input}} = f_{\text{integrate}}(I^*, T(t), S(s), C(c), E(e)) \]
1. \textbf{Integration Function \(f_{\text{integrate}}\)}: The integration function \(f_{\text{integrate}}\) merges the retrieved knowledge entry \(I^*\) with factors such as time, space, scenario, and energy to generate the decision input \(D_{\text{input}}\)：
\[ D_{\text{input}} = f_{\text{integrate}}(I^*, T(t), S(s), C(c), E(e)) \]
2. \textbf{Incorporation of Retrieved Knowledge into Decision Input}: The integration function \(f_{\text{integrate}}\) combines the retrieved knowledge entry \(I^*\) with factors including time, space, scenario, and energy to produce the decision input \(D_{\text{input}}\)：
\[ D_{\text{input}} = f_{\text{integrate}}(I^*, T(t), S(s), C(c), E(e)) \]
3. \textbf{Aggregation of Retrieved Knowledge with Time, Space, Scenario, and Energy by Integration Function \(f_{\text{integrate}}\)}: The integration function \(f_{\text{integrate}}\) consolidates the retrieved knowledge entry \(I^*\) with factors like time, space, scenario, and energy to generate the decision input \(D_{\text{input}}\)：
\[ D_{\text{input}} = f_{\text{integrate}}(I^*, T(t), S(s), C(c), E(e)) \]

其中：
\begin{itemize}
    \item \(T(t)\)表示时间因素。
    \item \(S(s)\)表示空间因素。
    \item \(C(c)\)表示场景因素。
    \item \(E(e)\)表示能量需求。
\end{itemize}
Where：
\begin{itemize}
    \item \(T(t)\) represents the time factor.
    \item \(S(s)\) represents the space factor.
    \item \(C(c)\) represents the scene factor.
    \item \(E(e)\) represents the energy demand.
\end{itemize}

\textbf{(4). Generation of electricity consumption behavior plan} \\
基于综合的决策输入\(D_{\text{input}}\)，用电行为计划生成函数\(f_{\text{plan}}\)用于生成具体的用电行为计划\(P\)：
\[ P = f_{\text{plan}}(D_{\text{input}}) \]
1. Based on the comprehensive decision input \(D_{\text{input}}\), the electricity behavior planning generation function \(f_{\text{plan}}\) is used to produce a specific electricity behavior plan \(P\):
\[ P = f_{\text{plan}}(D_{\text{input}}) \]
2. With the comprehensive decision input \(D_{\text{input}}\), the electricity behavior planning function \(f_{\text{plan}}\) is employed to generate a specific electricity behavior plan \(P\):
\[ P = f_{\text{plan}}(D_{\text{input}}) \]
3. Utilizing the comprehensive decision input \(D_{\text{input}}\), the function \(f_{\text{plan}}\) is utilized to create a specific electricity behavior plan \(P\) based on the input:
\[ P = f_{\text{plan}}(D_{\text{input}}) \]

\textbf{(5). Decision output and feedback} \\
决策输出\(D\)包括用电行为的时间、空间、场景、能量和价格等方面：
\[ D = [T(t), S(s), C(c), E(e), P(p)] \]
1. The decision output \(D\) includes aspects such as time, space, scenario, energy, and price related to electricity behavior:
\[ D = [T(t), S(s), C(c), E(e), P(p)] \]
2. The decision output \(D\) encompasses time, space, scenario, energy, and price aspects regarding electricity behavior:
\[ D = [T(t), S(s), C(c), E(e), P(p)] \]
3. The decision output \(D\) comprises elements involving time, space, scenario, energy, and price aspects of electricity behavior:
\[ D = [T(t), S(s), C(c), E(e), P(p)] \]

\noindent 通过实时反馈机制\(f_{\text{feedback}}\)，根据实际用电行为和环境变化调整决策生成函数：
\[ f_{\text{plan}}^{\text{new}} = f_{\text{feedback}}(f_{\text{plan}}, \text{actual\_behavior}, \text{environment\_changes}) \]
1. \noindent With the real-time feedback mechanism \(f_{\text{feedback}}\), the decision generation function is adjusted based on actual electricity behavior and environmental changes:
\[ f_{\text{plan}}^{\text{new}} = f_{\text{feedback}}(f_{\text{plan}}, \text{actual\_behavior}, \text{environment\_changes}) \]
2. \noindent Adjust the decision generation function \(f_{\text{plan}}^{\text{new}}\) based on actual electricity behavior and environmental changes through the real-time feedback mechanism \(f_{\text{feedback}}\):
\[ f_{\text{plan}}^{\text{new}} = f_{\text{feedback}}(f_{\text{plan}}, \text{actual\_behavior}, \text{environment\_changes}) \]
3. \noindent By utilizing the real-time feedback mechanism \(f_{\text{feedback}}\), the decision generation function is adapted according to actual electricity behavior and changes in the environment:
\[ f_{\text{plan}}^{\text{new}} = f_{\text{feedback}}(f_{\text{plan}}, \text{actual\_behavior}, \text{environment\_changes}) \]

% \textbf{(6). 综合检索增强过程} \\
% 整个检索增强过程可以表示为以下步骤：
% \begin{enumerate}
%     \item 构建和更新知识库：\[ K_{t+1} = K_t \cup \{(I_{N+1}, t_{N+1})\} \]
%     \item 从知识库中检索相关信息：\[ I^* = f_{\text{retrieve}}(K, q) \]
%     \item 整合检索信息和其他因素：\[ D_{\text{input}} = f_{\text{integrate}}(I^*, T(t), S(s), C(c), E(e)) \]
%     \item 生成用电行为计划：\[ P = f_{\text{plan}}(D_{\text{input}}) \]
%     \item 实施决策并监控实际行为和环境变化：\[ \text{monitor}(\text{actual\_behavior}, \text{environment\_changes}) \]
%     \item 根据反馈调整计划生成函数：\[ f_{\text{plan}}^{\text{new}} = f_{\text{feedback}}(f_{\text{plan}}, \text{actual\_behavior}, \text{environment\_changes}) \]
% \end{enumerate}



\section{基于生成式Agent模型实施：以电动汽车充电行为为例}
1. \textbf{Implementing Based on Generative Agent Model: Taking Electric Vehicle Charging Behavior as an Example}
2. \textbf{Implementation Using a Generative Agent Model: A Case Study of Electric Vehicle Charging Behavior}
3. \textbf{Execution Based on Generative Agent Model: Illustration with Electric Vehicle Charging Behavior}




\subsection{persona}
在模拟电动汽车充电行为的生成型Agent中，我们将设计多种角色（persona），以更好地反映不同用户群体的多样化行为。这些角色将包括以下属性：
人口统计信息：包括年龄、性别、职业等。这些信息可以影响用户的驾驶和充电行为。例如，年轻人可能更愿意接受新技术，更频繁地使用电动汽车和充电设施；而职业可能影响用户的行驶需求和充电时间。
经济条件：包括收入、财产等。这些信息可以影响用户的充电选择。例如，经济条件好的用户可能更愿意支付高价的快速充电服务。
车辆信息：包括电动汽车的型号、电池容量、能耗等。这些信息可以影响用户的充电需求和频率。
电动汽车充电心理信息：包括用户对电动汽车充电的认知、态度、意愿等。这些信息可以影响用户的充电行为和选择。
充电习惯：包括用户的充电频率、充电时间、充电地点选择等。这些信息可以影响用户的充电行为和充电站的使用情况。
通过模拟这些角色的充电行为，我们可以更全面地了解电动汽车用户的充电需求和习惯，从而为充电基础设施的规划和优化提供有力支持。
1. In the generative agent modeling of simulating electric vehicle charging behavior, we will design multiple personas to better reflect the diverse behaviors of different user groups. These roles will include the following attributes:
Demographic information: including age, gender, occupation, etc. These details can influence a user's driving and charging behavior. For example, younger individuals may be more inclined to adopt new technology, use electric vehicles and charging facilities more frequently; while occupation may affect a user's driving needs and charging times.
Economic conditions: including income, assets, etc. These details can impact a user's charging choices. For instance, users with better economic conditions may be more willing to pay for high-priced fast charging services.
Vehicle information: including the model, battery capacity, energy consumption, etc., of the electric vehicle. These details can influence a user's charging needs and frequency.
Psychological information related to electric vehicle charging: including the user's perception, attitude, willingness towards electric vehicle charging, etc. These details can affect a user's charging behavior and choices.
Charging habits: including the user's charging frequency, times, choice of charging locations, etc. These details can influence a user's charging behavior and the usage of charging stations. 
By simulating the charging behavior of these roles, we can better understand the charging needs and habits of electric vehicle users comprehensively, thereby providing strong support for the planning and optimization of charging infrastructure.
2. In the simulation of electric vehicle charging behavior using a generative agent model, we will create various personas to better represent the diverse behaviors of different user groups. These personas will encompass the following attributes:
Demographic information: including age, gender, occupation, and more. These details can impact a user's driving and charging behavior. For example, younger individuals may be more open to new technology and use electric vehicles and charging facilities more frequently, while occupation may influence a user's driving needs and charging times.
Economic status: including income, assets, and other factors. This information can affect a user's charging preferences. For instance, users with better economic conditions may be more willing to utilize high-priced fast charging services.
Vehicle details: such as the electric vehicle model, battery capacity, energy consumption, and other relevant information. These details can influence a user's charging demands and frequency.
Psychological aspects of electric vehicle charging: covering the user's perceptions, attitudes, willingness towards electric vehicle charging, and more. These aspects can impact a user's charging behaviors and choices.
Charging habits: including the user's charging frequency, timing, selection of charging locations, and more. These details can influence a user's charging behaviors and the utilization of charging stations. 
By simulating the charging behaviors of these personas, we can gain a more comprehensive understanding of electric vehicle users' charging needs and habits, thereby offering robust support for the planning and optimization of charging infrastructure.
3. In the implementation of a generative agent model to simulate electric vehicle charging behavior, we will design multiple personas to effectively capture the diverse behaviors of different user segments. These roles will include various characteristics such as:
Demographic information: encompassing age, gender, occupation, and other relevant factors. These details can impact a user's driving and charging patterns. For example, younger individuals might be more inclined to adopt new technologies, use electric vehicles and charging facilities more frequently, while occupation could influence driving requirements and charging schedules.
Economic circumstances: covering income, assets, and other financial aspects. These details can influence a user's charging preferences. For instance, users with better economic conditions may be more willing to pay for high-cost fast charging services.
Vehicle details: including the model, battery capacity, energy consumption, and other specifications of the electric vehicle. These details can impact a user's charging demands and frequency.
Psychological aspects related to electric vehicle charging: comprising a user's perceptions, attitudes, willingness towards electric vehicle charging, and other psychological factors. These aspects can affect a user's charging behavior and choices.
Charging habits: involving the user's charging frequency, timing, choice of charging locations, and other related behaviors. These details can influence a user's charging patterns and the utilization of charging stations.   
Through simulating the charging behaviors of these personas, we can gain a comprehensive understanding of electric vehicle users' charging needs and habits, thus providing valuable support for the planning and optimization of charging infrastructure.

\subsection{Planning}

在电动汽车充电行为的生成型Agent中，我们将设计以下几种计划模块：
1. In the generational Agent for electric vehicle charging behavior, we will design the following plan modules.
2. We will design several plan modules in the generative Agent for charging behavior of electric vehicles.
3. The design of various planning modules will be incorporated into the generative Agent for charging behaviors in electric cars.

\subsubsection{事件计划**}：Agent（在这里指电动汽车用户）会根据自己的日常活动安排，例如工作、购物、休闲等，来计划出行事件。每个事件可能会对电动汽车的行驶距离和充电需求产生影响。   
\subsubsection{Event Planning**}: Agents (referring to electric vehicle users in this context) will organize their travel events based on their daily activities such as work, shopping, leisure, etc. Each event may impact the driving range and charging requirements of electric vehicles.
\subsubsection{Event Planning**}: Agents (here referring to electric car users) will plan their travel events based on their daily activities such as work, shopping, leisure, etc. Each event may affect the driving distance and charging needs of electric cars.
\subsubsection{Event Planning**}: Agents (referring to electric car users here) will schedule their travel events based on their daily activities like work, shopping, leisure, etc. Each event might influence the driving range and charging demands of electric cars.

\subsubsection{出行计划**}- ****：基于事件计划，Agent会进一步规划出行路线和时间。例如，Agent可能会选择最短路线或者最省电路线，也可能会选择在交通流量较小的时段出行。 
\subsubsection{Travel Planning**} - ****: Building upon the event plan, Agents will further plan their travel routes and timing. For instance, Agents may opt for the shortest route or the most energy-efficient route, and they may also choose to travel during off-peak traffic hours.
\subsubsection{Travel Planning**} - ****: Based on the event plan, Agents will proceed to map out their travel routes and schedule. For example, Agents may select the shortest route or the most economical in terms of energy consumption, and they may also choose to travel during periods of lighter traffic flow.
\subsubsection{Travel Planning**} - ****: Expanding on the event plan, Agents will then proceed to organize their travel routes and timing. They may opt for the shortest route or the most fuel-efficient route, and they may also select travel times with lower traffic congestion.

\subsubsection{出行时间和距离**}：这是出行计划的一部分，Agent会预估每次出行的时间和距离。出行时间和距离将直接影响电动汽车的电量消耗。
\subsubsection{Travel Time and Distance**}: This is a part of the travel plan where Agents will estimate the time and distance for each journey. The travel time and distance will directly impact the energy consumption of the electric vehicle.
\subsubsection{Travel Time and Distance**}: As a component of the travel plan, Agents will predict the time and distance for each trip. The travel duration and distance will have a direct impact on the energy consumption of the electric vehicle.
\subsubsection{Travel Time and Distance**}: Forming part of the travel plan, Agents will project the time and distance for each journey. These factors will directly influence the energy consumption of the electric vehicle.

\subsubsection{充电计划**}：基于出行计划和电动汽车的电量状态，Agent会规划充电行为。例如，Agent可能会选择在电量低于一定阈值时进行充电，或者在到达目的地附近有充电站的情况下进行充电。充电计划也会考虑到充电站的位置、充电速度和费用等因素。
1.\subsubsection{Charging Plan**}: Based on the travel plan and the battery status of the electric vehicle, Agents will strategize their charging behavior. For instance, Agents may choose to charge when the battery level drops below a certain threshold, or when there are charging stations near the destination. The charging plan will also take into account factors such as the location of charging stations, charging speed, and costs.
2.\subsubsection{Charging Plan**}: Drawing from the travel plan and the electric car's battery status, Agents will devise a charging strategy. For example, Agents may opt to charge when the battery level falls below a specific threshold, or when near a destination with available charging stations. The charging plan will also account for factors like the location of charging stations, charging speed, and costs.
3.\subsubsection{Charging Plan**}: Based on the travel plan and the electric vehicle's battery status, Agents will plan their charging activities. For example, Agents may choose to charge when the battery level is below a certain threshold, or when there are charging stations near the destination. The charging plan will also consider factors such as the location of charging stations, charging speed, and costs.

这些计划模块将帮助Agent更有效地管理电动汽车的电量，满足出行需求，同时也能够优化充电行为，提高充电效率和用户满意度。
1.These planning modules will assist Agents in more effectively managing the electric vehicle's battery power to meet travel needs, as well as optimize charging behavior to enhance charging efficiency and user satisfaction.
2.These planning modules will help Agents manage the electric vehicle's battery more effectively to meet travel requirements, and also optimize charging behaviors to improve charging efficiency and user satisfaction.
3.These planning modules will aid Agents in managing the electric vehicle's battery more efficiently to satisfy travel demands, and also optimize charging practices to boost charging effectiveness and user satisfaction.

\subsection{Observation}
在电动汽车充电行为的生成型Agent中，我们将设计以下几种感知模块：
1.In the generative Agent for electric vehicle charging behavior, we will design the following perception modules:
2.In the generative Agent for electric vehicle charging behavior, the following perception modules will be designed:
3.In the generative Agent for electric vehicle charging behavior, we will incorporate the following perception modules:

\subsubsection{Vehicle Perception：}
The Agent (referring to the electric vehicle here) is able to perceive the following information:
\begin{itemize}
    \item 出行时间：车辆能够记录每次出行的时间，这对于预测电量消耗和规划充电行为非常重要。
    1. \item Travel Time Recording: The vehicle can record the time of each trip, which is crucial for predicting power consumption and planning charging activities.
    2. \item Time Tracking for Travel: The vehicle has the capability to track the duration of every trip, which is essential for estimating energy usage and scheduling charging activities.
    3. \item Time Recording for Journeys: The vehicle is able to log the time taken for each journey, a key factor for forecasting energy consumption and organizing charging routines.
    
    \item 出行距离：车辆能够记录每次行驶的距离，这也是预测电量消耗和规划充电行为的重要信息。
    1.\item  Travel Distance Recording: The vehicle can record the distance traveled on each trip, which is vital for predicting power consumption and planning charging activities.
    2.\item  Distance Tracking for Travel: The vehicle is capable of tracking the distance covered during every journey, which is crucial for estimating energy usage and organizing charging routines.
    3.\item  Distance Recording for Journeys: The vehicle can log the distance traveled for each trip, providing essential information for forecasting energy consumption and scheduling charging behaviors.
    
    \item 现有能量：车辆能够实时监测电池的剩余电量，当电量低于一定阈值时，车辆需要进行充电。
    1. \item Real-time Energy Status: The vehicle can monitor the remaining battery level in real-time. When the energy level falls below a certain threshold, the vehicle needs to be charged.
    2. \item Current Energy Level: The vehicle has the capability to continuously monitor the battery's remaining energy level. Charging is required when the energy level drops below a set threshold.
    3. \item Available Energy: The vehicle is able to monitor the real-time energy level of the battery. When the energy level falls below a specific threshold, the vehicle needs to undergo charging.
    
    \item 能量消耗：车辆能够计算每次行驶消耗的电量，这有助于更准确地预测电量需求和规划充电行为。
    1.\item Energy Consumption Calculation: The vehicle can calculate the amount of electricity consumed during each trip, which helps in more accurately predicting energy needs and planning charging activities.
    2.\item Calculating Energy Usage: The vehicle has the ability to compute the electricity consumed on each journey, aiding in precise forecasting of energy requirements and scheduling charging routines.
    3.\item Energy Expenditure Measurement: The vehicle can determine the electric power consumed during each trip, enhancing the accuracy of energy demand predictions and charging plans.
    
\end{itemize}


\subsubsection{Charging station perception：}
The Agent can also perceive the following information about the charging station
：
\begin{itemize}
    \item 充电排队情况：Agent能够获取充电站的实时排队情况，这对于规划充电行为和预测充电等待时间非常重要。
    1.\item Real-time Charging Queue Status: The agent is able to gather up-to-date information on the queue status at charging stations, which is essential for planning charging activities and predicting charging wait times.
    2.\item Current Charging Station Queue Status: The agent can retrieve real-time data on the queue situation at charging stations, which plays a vital role in organizing charging activities and estimating charging wait times.
    3.\item Charging Station Queue Monitoring: The agent has the capability to monitor the real-time queue status at charging stations, which is crucial for planning charging activities and forecasting charging wait times.
    
    \item 距离：Agent能够计算到最近充电站的距离，这有助于规划充电行为和预测电量需求。
    1.\item Distance Calculation to Nearest Charging Station: The agent can calculate the distance to the nearest charging station, which is beneficial for planning charging activities and predicting energy requirements.
    2.\item Determining Distance to Closest Charging Station: The agent has the ability to compute the distance to the nearest charging station, aiding in the planning of charging activities and forecasting energy demands.
    3.\item Distance to Nearest Charging Point Calculation: The agent can determine the distance to the closest charging station, which helps in planning charging behaviors and predicting energy needs.
    
    \item 充电功率：Agent能够获取充电站的充电功率，这对于预测充电时间非常重要。
    1.\item Charging Power: The agent can access the charging power of charging stations, which is crucial for predicting charging times.
    2.\item Power Information at Charging Stations: The agent is able to obtain the charging power available at charging stations, which is essential for accurate prediction of charging times.
    3.\item Charging Station Power Capacity: The agent can retrieve information on the charging power capacity at charging stations, which is vital for accurately predicting charging times.
    
    \item 充电价格：Agent能够获取充电站的充电价格，这对于用户来说是选择充电站的重要因素。
    1.\item Charging Prices: The agent can access the charging prices at charging stations, which are important factors for users when selecting a charging station.
    2.\item Price Information at Charging Stations: The agent is able to retrieve the charging prices at charging stations, which is a crucial factor for users in choosing a charging station.
    3.\item Charging Station Pricing: The agent can obtain the charging prices at charging stations, which is an important consideration for users when selecting a charging station.
\end{itemize}

这些感知模块将帮助Agent更准确地理解自身的状态和环境，以便做出更好的决策。
1. These perception modules will assist the agent in better understanding its own state and environment, enabling it to make more informed decisions.
2. By utilizing these perception modules, the agent will be able to accurately comprehend its status and surroundings, leading to improved decision-making.
3. The utilization of these perception modules will aid the agent in gaining a more precise understanding of its own state and the environment, facilitating enhanced decision-making.

\subsection{memory}


为了更好地模拟电动汽车用户的充电行为，我们的生成型Agent需要具备记忆功能，以记录和管理过去的充电数据。记忆设计主要包括短期记忆和长期记忆两部分。
1. In order to better simulate the charging behavior of electric vehicle users, our generative agent needs to have memory capabilities to store and manage past charging data. The memory design mainly includes short-term memory and long-term memory.
2. To enhance the simulation of electric vehicle users' charging behavior, our generative agent must possess memory functions to store and manage historical charging data. The memory design primarily consists of short-term memory and long-term memory.
3. To improve the modeling of electric vehicle users' charging behaviors, our generative agent requires memory functionality to capture and manage past charging data effectively. The memory design encompasses both short-term memory and long-term memory capabilities.

\subsubsection{短期记忆} 短期记忆主要记录最近三天内的充电行为数据，包括充电时间、充电站、充电量、充电功率和充电价格。这些数据可以帮助Agent在短期内做出更合理的决策。例如，如果Agent记住了最近几天内充电站的排队情况，那么它就可以在选择充电站时避开高峰时段，从而节省充电等待时间。
1. \subsubsection{Short-term Memory}: The short-term memory primarily stores charging behavior data from the past three days, including charging time, charging station, charging amount, charging power, and charging prices. These data can assist the agent in making more informed decisions in the short term. For example, if the agent remembers the queue situation at charging stations in recent days, it can avoid peak hours when selecting a charging station, thereby saving charging waiting time.
2. \subsubsection{Short-Term Memory Function}: The short-term memory function is responsible for storing charging behavior data from the last three days, such as charging time, charging station, charging amount, charging power, and charging prices. This information enables the agent to make more rational decisions in the short term. For instance, by remembering the recent queue situation at charging stations, the agent can choose a time to charge that avoids peak hours, thus reducing charging wait times.
3.\subsubsection{Recording Short-Term Memory}: The short-term memory module records charging behavior data from the past three days, including details like charging time, charging station, charging amount, charging power, and charging prices. This data equips the agent to make more reasonable decisions in the short term. For instance, if the agent recalls the recent queue status at charging stations, it can select times to charge that steer clear of peak periods, ultimately saving on charging wait times.

\subsubsection{长期记忆} 长期记忆主要记录最近七天内的充电行为数据，包括充电时间、充电站、充电量、充电功率和充电价格。这些数据可以帮助Agent在长期内分析用户的充电习惯和趋势，从而进行更好的行为规划和决策。例如，如果Agent记住了用户在工作日和周末的充电行为有显著差异，那么它就可以据此调整自己的充电计划，以更好地满足用户的需求。
1. \subsubsection{Long-term Memory}: The long-term memory primarily stores charging behavior data from the past seven days, including charging time, charging station, charging amount, charging power, and charging prices. This data can help the agent analyze users' charging habits and trends over the long term, facilitating better behavior planning and decision-making. For example, if the agent remembers significant differences in user charging behavior between weekdays and weekends, it can adjust its charging plan accordingly to better meet users' needs.
2.\subsubsection{Long-Term Memory Function}: The long-term memory function is responsible for storing charging behavior data from the past seven days, encompassing details like charging time, charging station, charging amount, charging power, and charging prices. This data enables the agent to analyze users' charging habits and trends over an extended period, leading to enhanced behavior planning and decision-making. For instance, by retaining information on distinct user charging patterns during weekdays and weekends, the agent can adapt its charging schedule to better cater to user requirements.
3.\subsubsection{Recording Long-Term Memory}: The long-term memory module records charging behavior data from the last seven days, including charging time, charging station, charging amount, charging power, and charging prices. This data facilitates the agent in analyzing user charging habits and trends over a longer period, enabling improved behavior planning and decision-making. For example, if the agent remembers significant differences in user charging behavior between weekdays and weekends, it can adjust its charging schedule accordingly to better meet user needs.

此外，我们的记忆设计也会考虑到记忆的相关性、重要性和时效性，以便更有效地管理和检索记忆。例如，Agent可能会优先记住和当前情境相关的信息，或者优先记住对决策影响较大的信息。同时，Agent也会定期更新自己的记忆，以保证记忆的时效性。
1. In addition, our memory design also takes into account the relevance, importance, and timeliness of memories to effectively manage and retrieve information. For instance, the agent may prioritize remembering information that is relevant to the current context or information that has a significant impact on decision-making. Simultaneously, the agent will regularly update its memory to ensure its timeliness.
2. Furthermore, our memory design considers the relevance, importance, and timeliness of memories to enhance memory management and retrieval efficiency. For example, the agent may prioritize remembering information relevant to the current situation or information crucial for decision-making. Additionally, the agent periodically updates its memory to maintain its relevance.
3. Additionally, our memory design will take into consideration the relevance, importance, and timeliness of memories to efficiently manage and retrieve memories. For instance, the agent may prioritize remembering information that is related to the current context or information that significantly influences decision-making. At the same time, the agent will update its memory regularly to ensure its timeliness.

\subsection{（Decision Making）}

在电动汽车充电行为的生成型Agent中，我们将设计以下决策模块：
1. Charging Behavior Generation Agent: In the context of electric vehicle charging behavior, we will design the following decision modules:
2. Decision Module Design for Electric Vehicle Charging Behavior Generation Agent: Within the framework of an electric vehicle charging behavior generation agent, we will develop the following decision modules:
3. Decision Module Design for Electric Vehicle Charging Behavior Generating Agent: In the realm of electric vehicle charging behavior generation, we will establish the following decision modules:

决策模块需要根据角色（电动汽车用户）、事件计划（例如出行计划和充电计划）、记忆（例如过去的充电行为数据）和感知信息（例如车辆状态和充电站情况），来做出合理的决策。具体的决策内容包括：
1. The decision module needs to make reasonable decisions based on roles (electric vehicle users), event plans (such as travel and charging schedules), memory (such as past charging behavior data), and sensory information (such as vehicle status and charging station conditions). Specific decision content includes:
2. The decision module is required to make informed decisions based on roles (electric vehicle users), event schedules (such as travel plans and charging schedules), memory (e.g., past charging behavior data), and sensory information (e.g., vehicle status and charging station conditions). The specific decision-making content includes:
3. The decision module must make rational decisions based on roles (electric vehicle users), event plans (e.g., travel plans and charging plans), memory (e.g., past charging behavior data), and sensory information (e.g., vehicle status and charging station conditions). The specific decision content includes:

\subsubsection{充电时间}
根据电动汽车的电量状态、出行计划和充电站的排队情况，决定合适的充电时间。例如，如果电量低于一定阈值，且充电站当前没有排队，那么现在就是一个好的充电时间。
1.\subsubsection{Charging Time}
Decide on the appropriate charging time based on the electric vehicle's battery status, travel plans, and the queue situation at charging stations. For example, if the battery level is below a certain threshold and there is no queue at the charging station, then now would be a good time to charge.
2.\subsubsection{Charging Time}
Determine the suitable charging time considering the electric vehicle's battery level, travel plans, and the queuing situation at charging stations. For instance, if the battery level falls below a specific threshold and there is no queue at the charging station, it is an opportune time to charge.
3.\subsubsection{Charging Time}
Decide on the appropriate charging time based on the electric car's battery level, travel plans, and the queue status at charging stations. For example, if the battery level is below a certain threshold and there is no queue at the charging station, then it is a good time to charge.

\subsubsection{充电站选择}根据充电站的位置、充电功率、充电价格和排队情况，选择最合适的充电站。例如，如果某个充电站离用户的目的地近，充电速度快，价格合理，且没有排队，那么这个充电站就是一个好的选择。
1.\subsubsection{Charging Station Selection}
Choose the most suitable charging station based on the location, charging power, pricing, and queue status of the charging stations. For example, if a charging station is close to the user's destination, offers fast charging, reasonable pricing, and has no queue, then this charging station is a good choice.
2.\subsubsection{Choosing a Charging Station}
Select the optimal charging station by considering its location, charging power, pricing, and queue status. For instance, if a charging station is close to the user's destination, provides fast charging, offers reasonable prices, and has no queue, then it is a good choice.
3.\subsubsection{Charging Station Selection}
Based on the location, charging power, pricing, and queue status of charging stations, choose the most suitable one. For example, if a charging station is close to the user's destination, has fast charging speed, reasonable pricing, and no queue, then it is a good choice.

\subsubsection{充电量} 根据电动汽车的电量状态和出行计划，决定需要充电的电量。例如，如果电动汽车的电量已经很低，且用户明天需要长途出行，那么可能需要充满电。
1.\subsubsection{Charging Amount}
Determine the required amount of charge based on the electric vehicle's battery status and travel plans. For example, if the electric vehicle's battery level is already very low and the user has a long trip planned for tomorrow, it may be necessary to fully charge it.
2.\subsubsection{Battery Charging}
Decide on the amount of charge needed based on the electric vehicle's battery status and travel plans. For instance, if the electric vehicle has a very low battery level and the user has a long trip scheduled for tomorrow, it may be necessary to charge it fully.
3.\subsubsection{Charging Quantity}
Decide on the required charging amount based on the electric car's battery status and travel plans. For example, if the electric car's battery level is very low and the user has a long trip planned for tomorrow, it may be necessary to charge it to full capacity.

\subsubsection{充电功率} 根据电动汽车的电量状态和充电站的充电功率，决定使用的充电功率。例如，如果电量很低，且充电站的充电功率高，那么可以选择高功率充电，以节省充电时间。
1.\subsubsection{Charging Power}
Decide on the charging power to use based on the electric vehicle's battery status and the charging station's power. For example, if the battery level is very low and the charging station has high power, opting for high-power charging can save charging time.
2.\subsubsection{Power Rating for Charging}
Choose the appropriate charging power based on the electric vehicle's battery status and the charging station's power rating. For instance, if the battery level is very low and the charging station offers a high power rating, selecting high-power charging can help save charging time.
3.\subsubsection{Charging Power Level}
Based on the electric car's battery status and the charging station's power rating, determine the appropriate charging power level to use. For example, if the battery level is very low and the charging station provides high power, opting for high-power charging can help reduce charging time.

\subsubsection{充电价格} 根据充电站的充电价格和用户的支付意愿，决定是否接受这个价格。例如，如果充电价格高于用户的预期，那么用户可能会选择其他更便宜的充电站。
1.\subsubsection{Charging Price}
Decide whether to accept the charging price based on the charging station's rates and the user's willingness to pay. For example, if the charging price is higher than the user's expectations, they may opt for a cheaper charging station.
2.\subsubsection{Pricing for Charging}
Based on the charging station's rates and the user's willingness to pay, determine whether to accept the price. For instance, if the charging price exceeds the user's expectations, they may choose a more affordable charging station instead.
3.\subsubsection{Charging Station Fees}
Consider the charging station's pricing and the user's payment preferences to decide on accepting the price. For example, if the charging fees are higher than expected by the user, they might opt for a different, more cost-effective charging station.

这些决策将帮助Agent更有效地管理电动汽车的电量，满足用户的出行和充电需求，同时也能够优化充电行为，提高用户满意度。
1.These decisions will help the agent to effectively manage the electric vehicle's battery level, meet the users' travel and charging needs, optimize charging behavior, and enhance user satisfaction.
2.These decisions will assist the agent in managing the electric vehicle's battery level more effectively, meeting users' travel and charging requirements, optimizing charging behavior, and increasing user satisfaction.
3.These decisions will aid the agent in efficiently managing the electric vehicle's battery level, fulfilling users' travel and charging needs, optimizing charging behavior, and improving user satisfaction.

\subsection{Reflection}
反思是一个重要的环节，它有助于Agent识别和改进决策中的不足之处，从而优化未来的充电行为。具体来说，反思模块可能包括以下几个部分：
1.Reflection is a crucial step that helps the agent identify and improve deficiencies in decision-making, thereby optimizing future charging behaviors. Specifically, the reflection module may include the following components:
2.Reflection is a critical stage that aids the agent in recognizing and enhancing shortcomings in decision-making, leading to the optimization of future charging behaviors. In particular, the reflection module may consist of the following parts:
3.Reflection is an important aspect that assists the agent in identifying and improving shortcomings in decision-making, thus optimizing future charging behaviors. More specifically, the reflection module may encompass the following components:

\subsubsection{计划匹配} Agent需要评估所做决策是否准确地满足了用户的需求和期望。例如，Agent可以反思用户是否在计划的时间内成功完成充电，以此来评估决策的准确性。
1.\subsubsection{Plan Matching} The agent needs to assess whether the decisions made accurately meet the users' needs and expectations. For example, the agent can reflect on whether the user successfully completed charging within the planned time to evaluate the decision's accuracy.
2.\subsubsection{Plan Matching} The agent must evaluate whether the decisions accurately met the users' needs and expectations. For instance, the agent could reflect on whether the user successfully completed charging within the planned time frame to assess the decision's accuracy.
3.\subsubsection{Plan Matching} The agent has to evaluate whether the decisions accurately met the users' needs and expectations. For instance, the agent could reflect on whether the user successfully completed charging within the planned time frame to assess the decision's accuracy.

\subsubsection{用户满意度} Agent需要评估用户对充电决策的满意度，包括充电时间、充电站选择、充电量、充电功率和充电价格等方面。例如，Agent可以通过用户对充电时间的满意度评分（例如4/5）来反思自己的决策。
1.\subsubsection{User Satisfaction} The agent needs to assess user satisfaction with charging decisions, including aspects such as charging time, charging station selection, charging amount, charging power, and charging price. For example, the agent can reflect on their decisions by evaluating user satisfaction ratings for charging time (e.g., 4/5).
2.\subsubsection{User Satisfaction} The agent must evaluate user satisfaction with charging decisions, encompassing factors like charging time, choice of charging station, charging amount, charging power, and charging cost. For instance, the agent could assess their decisions by reflecting on user satisfaction ratings for charging time (e.g., 4/5).
3.\subsubsection{User Satisfaction} The agent has to assess user satisfaction with charging decisions, covering aspects such as charging time, selection of charging station, amount of charge, charging power, and charging price. For example, the agent can reflect on their decisions by considering user satisfaction scores for charging time (e.g., 4/5).

\subsubsection{成本效益} Agent需要评估充电决策的成本效益，包括充电费用和时间成本。例如，Agent可以反思充电费用是否在用户可接受的范围内，充电时间是否合理，以此来评估决策的成本效益。
1.\subsubsection{Cost-effectiveness} The agent needs to evaluate the cost-effectiveness of charging decisions, including charging costs and time costs. For example, the agent can reflect on whether the charging costs fall within the range acceptable to users, and whether the charging time is reasonable, to assess the cost-effectiveness of decisions.
2.\subsubsection{Cost-Benefit Analysis} The agent is required to assess the cost-effectiveness of charging decisions, which includes charging fees and time costs. For instance, the agent may reflect on whether the charging fees are within the acceptable range for users and if the charging time is reasonable, in order to evaluate the cost-effectiveness of the decisions.
3.\subsubsection{Cost-benefit Evaluation} The agent needs to evaluate the cost-effectiveness of charging decisions, which involves assessing charging fees and time costs. For example, the agent can reflect on whether the charging fees are within the acceptable range for users and if the charging time is reasonable, as a way to evaluate the cost-effectiveness of decisions.

通过反思，Agent可以从过去的经验中学习，不断优化自己的行为和决策，从而更好地满足用户的充电需求。
1. Through reflection, the agent can learn from past experiences to continuously optimize its actions and decisions, thereby better meeting users' charging needs.
2. By reflecting, the agent can learn from past experiences to constantly improve its behavior and decisions, thus better catering to users' charging requirements.
3. Through reflection, the agent can learn from past experiences to repeatedly enhance its actions and decisions, in order to better fulfill users' charging demands.

\section{Interactive design of simulation environment}

通过这样的环境交互设计，我们可以模拟电动汽车用户的充电行为，以及这些行为如何影响电动汽车和充电站的状态。这将有助于我们理解和预测电动汽车的充电需求。
1. Through this type of environmental interaction design, we can simulate the charging behavior of electric vehicle users and how these behaviors impact the states of electric vehicles and charging stations. This will help us understand and predict the charging needs of electric vehicles.
2. By employing such environmental interaction design, we can replicate the charging behaviors of electric vehicle users and study how these behaviors influence the statuses of both electric vehicles and charging stations. This will aid us in comprehending and forecasting the charging requirements of electric vehicles.
3. This environmental interaction design allows us to simulate the charging behaviors of electric vehicle users and how these behaviors affect the statuses of electric vehicles and charging stations. This simulation approach can enhance our understanding and prediction of the charging demands of electric vehicles.
在仿真设计中，我们将模拟电动汽车用户的充电行为，以及这些行为如何影响电动汽车和充电站的状态。我们将设定每15分钟仿真一次，这意味着，每15分钟，电动汽车用户都会根据当前的环境状态和自身的状态，做出决策，并执行相应的行为。
1. In the simulation design, we will simulate the charging behavior of electric vehicle users and how these behaviors impact the states of electric vehicles and charging stations. We will set the simulation to run every 15 minutes, which means that every 15 minutes, electric vehicle users will make decisions based on the current environmental conditions and their own states, and carry out corresponding actions.
2. Within the simulation design, we plan to mimic the charging behavior of electric vehicle users and examine how these actions influence the statuses of electric vehicles and charging stations. The simulation will be conducted in 15-minute intervals, indicating that every 15 minutes, electric vehicle users will make decisions and undertake relevant actions based on the prevailing environmental conditions and their own circumstances.
3. Through the simulation design, we aim to model the charging behavior of electric vehicle users and analyze the impact of these behaviors on the states of electric vehicles and charging stations. The simulation will run every 15 minutes, enabling electric vehicle users to make decisions and engage in appropriate actions according to the current environmental conditions and their personal statuses.
代理人与环境交互：在电动汽车充电行为的生成型Agent模型中，代理人（电动汽车用户）会根据环境信息（如电动汽车的电量、充电站的状态、价格等）做出是否充电的决策。此外，代理人还会根据他们的经验和记忆来计划他们的行为。例如，如果他们记住在特定时间（如晚上）充电更便宜，他们可能会计划在这个时间去充电。
1. Agent-Environment Interaction: In the generative Agent model of electric vehicle charging behavior, agents (electric vehicle users) make decisions on whether to charge based on environmental information (such as the battery level of electric vehicles, the status of charging stations, prices, etc.). Additionally, agents will plan their actions based on their experiences and memories. For example, if they recall that charging is cheaper at specific times (e.g., at night), they may plan to charge at that time.
2. Interaction between Agents and the Environment: In the generative Agent model of electric vehicle charging behavior, agents (electric vehicle users) decide whether to charge based on environmental information (e.g., the battery level of electric vehicles, charging station status, pricing, etc.). Furthermore, agents rely on their experiences and memories to plan their behavior. For instance, if they remember that charging is more affordable at certain times (like at night), they may schedule their charging for those times.
3. Agent-Environment Interaction: Within the generative Agent model of electric vehicle charging behavior, agents (electric vehicle users) make charging decisions based on environmental cues (such as electric vehicle battery levels, charging station statuses, prices, etc.). Moreover, agents employ their experiences and memories to plan their actions. For instance, if they recollect that charging is cheaper at specific times (e.g., at night), they might plan to charge during those periods.

\subsection{Electric vehicle users}
他们是代理人，根据电动汽车的电量、充电站的状态（如空闲的充电桩数量、价格等）、自身的需求（如行驶距离等），以及他们的经验和记忆，做出是否去充电、何时充电、在哪里充电等决策。
1. They are agents who make decisions on whether to charge, when to charge, and where to charge based on the electric vehicle's battery level, charging station status (such as the number of available charging spots, prices, etc.), their own needs (such as driving distance), as well as their experiences and memories.
2. These agents make decisions on whether to charge, when to charge, and where to charge by considering factors such as the electric vehicle's battery level, charging station status (including the availability of charging spots and pricing), their own requirements (such as driving distance), and drawing upon their experiences and memories.
3. Acting as agents, they determine whether to charge, when to charge, and where to charge based on the electric vehicle's battery level, the status of charging stations (such as the availability of charging spots, pricing, etc.), their own needs (such as driving distance), and their accumulated experiences and memories.

\subsection{电动汽车} 电动汽车是代理人行为的主要驱动因素。我们需要考虑电动汽车的电量、电池容量、充电速度、行驶距离等属性。这些属性将影响电动汽车用户的充电决策和行为。
1. \subsection{Electric Vehicles} Electric vehicles serve as the primary driving force behind agent behavior. Factors such as electric vehicle battery level, battery capacity, charging speed, and driving range need to be taken into account. These attributes play a significant role in shaping the charging decisions and actions of electric vehicle users.
2. \subsection{Electric Vehicles} Electric vehicles serve as the primary motivators for agent behavior. Consideration must be given to attributes such as electric vehicle battery level, battery capacity, charging speed, and driving range. These attributes have an impact on the charging decisions and behaviors of electric vehicle users.
3. \subsection{Electric Vehicles} Electric vehicles are the key drivers of agent behavior. Factors such as electric vehicle battery level, battery capacity, charging speed, and driving distance need to be considered. These attributes affect the charging decisions and behaviors of electric vehicle users.

\subsection{充电站} 充电站是电动汽车充电的主要环境。我们需要考虑充电站的位置、数量、充电桩的数量和类型（如快充、慢充）、价格、等待时间等因素。充电站的这些属性将影响电动汽车用户的充电决策和行为。
1. \subsection{Charging Stations} Charging stations form the primary environment for electric vehicle charging. Factors to consider include the location, quantity, number and types of charging ports (such as fast-charging, slow-charging), prices, waiting times, and other factors. These attributes of charging stations will impact the charging decisions and behaviors of electric vehicle users.
2. \subsection{Charging Stations} Charging stations serve as the main environment for electric vehicle charging. It is essential to take into account factors such as the location, quantity, types of charging ports (e.g., fast-charging, slow-charging), prices, waiting times, and other factors of the charging stations. These attributes of charging stations will influence the charging decisions and behaviors of electric vehicle users.
3. \subsection{Charging Stations} Charging stations are the primary infrastructure for electric vehicle charging. Considerations need to be made regarding the location, quantity, types of charging ports (e.g., fast-charging, slow-charging), prices, waiting times, and other factors of the charging stations. These attributes of charging stations will impact the charging decisions and behaviors of electric vehicle users.





% \section*{参考文献}
% \bibliographystyle{gbt7714-numerical}
\bibliographystyle{plain}
\bibliography{ref.bib}
\end{document}



